Effective Representations of Clinical Notes

Clinical notes are a rich source of information about patient state. However, using them to predict clinical events with machine learning models is challenging. They are very high dimensional, sparse and have complex structure. Furthermore, training data is often scarce because it is expensive to obtain reliable labels for many clinical events. These difficulties have traditionally been addressed by manual feature engineering encoding task specific domain knowledge. We explored the use of neural networks and transfer learning to learn representations of clinical notes that are useful for predicting future clinical events of interest, such as all causes mortality, inpatient admissions, and emergency room visits. Our data comprised 2.7 million notes and 115 thousand patients at Stanford Hospital. We used the learned representations, along with commonly used bag of words and topic model representations, as features for predictive models of clinical events. We evaluated the effectiveness of these representations with respect to the performance of the models trained on small datasets. Models using the neural network derived representations performed significantly better than models using the baseline representations with small ($N < 1000$) training datasets. The learned representations offer significant performance gains over commonly used baseline representations for a range of predictive modeling tasks and cohort sizes, offering an effective alternative to task specific feature engineering when plentiful labeled training data is not available.

==> sections/background.tex <==
Clinical text is one of the richest sources of information about
patients and health care that can be found in EHRs.  Researchers
utilize the text in clinical notes for a variety of applications:
phenotyping \citep{ford2016text,agarwal2016learning},
pharmacovigilance \citep{lependu2013pharmacovigilance,harpaz2014text},
and modeling risk \citep{ghassemi2014unfolding,halpern2012comparison}.
A number of studies have shown that adding text as an input alongside
physiologic measurements boosts the performance of clinical prediction
models by significant
margins \citep{ghassemi2014unfolding,caballero2015dynamically}.

The standard representation for clinical text is bag of words (BOW),
which represents a document as counts over a predefined vocabulary.
BOW is intuitive and easy to construct and manipulate.  It admits
simple heuristics for dimensionality reduction (e.g., discarding words
that are too frequent or infrequent) and schemes for incorporating
information about relative frequency, e.g., TF-IDF.
%BOW has enjoyed widespread success within health care~\citep{} and
%without~\citep{}.
However, BOW fails to fully address many of the challenges presented
by clinical text, leading health informatics researchers to seek
alternatives~\citep{halpern2012comparison,jung2015functional,choi2016learning,miotto2016deep}.

First, \textit{clinical notes are intrinsically high dimensional} due
to their diversity of topics, specialized vocabulary, and
combinatorial nature.  Naive representations such as BOW can yield
input (feature) vectors with hundreds of thousands of dimensions.
Patient cohorts, on the other hand, commonly number in the tens to
hundreds, even at hospitals with millions of digital records.
% \footnote{This is due in part to the fact that many clinical
% research questions define strict case and control definitions,
% limiting the number of patients available for inclusion in any
% one study. However, there is also a dearth of labeled data in EHRs:
% many outcomes of interest, such as mortality, occur outside the
% hospital and are not observed. Many diseases go undiagnosed for
% long periods of time, and many more diagnoses are not recorded
% in a consistent manner during the delivery of care.}
This invokes the ``curse of dimensionality,'' making statistical
models difficult to train without aggressive dimensionality reduction
or regularization.

In a related problem, \textit{clinical text data are also inherently
sparse}: phrases describing important clinical concepts may occur in
only a handful of records.  This makes it difficult to discover a
reliable statistical relationship between an outcome and such phrases,
as well as the concepts they denote.  This problem is exacerbated
by \textit{noise and ambiguity in clinical text}: ``tachycardia'' may
alternatively be described as a ``rapid heart rate'' or
``arrhythmia.''
% \footnote{Alternatively, a clinician may simply imply the presence
% of tachycardia by listing an obviously abnormal heart rate,
% trusting an expert reader will recognize it.}
One can easily imagine cases where the common BOW dimensionality
reduction heuristic of discarding rare terms actually removes all
mentions of an important concept.

\textit{Clinical notes also exhibit a hierarchical sequential
structure}: a longitudinal patient record includes a time series of
notes, each itself consisting of a sequence of words.
% Both types of sequences can have arbitrary length, and
This poses a trade-off between simplicity and fidelity when choosing a
representation: directly modeling this ``sequence of sequences''
structure requires a complex model architecture and most likely a
large amount of training data.  In contrast, representing a patient
history as a BOW is simple and flexible but discards information about
time and order.  There is a spectrum of choices between these
extremes, but they often involve only slightly less
complexity \citep{choi2015doctor} or ad hoc decisions about, e.g.,
windowing time \citep{schuler2016discovering}.

In this paper, we present two methods for representing clinical text
that occupy different points on the simplicity-richness spectrum.  We
evaluate the representations within the framework of transfer
learning \textemdash we first learn how to represent patients using
a \emph{source task} with no or relatively plentiful labels, and then
use the learned representations for new \emph{target tasks} in which
we learn to predict future events from small training samples.  The
resulting models are then evaluated on held out test patients.  The
first method, \emph{embed-and-aggregate}, is very simple and requires
no external labels for supervision.  The second method uses recurrent
neural nets to explicitly model the sequential nature of the notes,
and is supervised using labels derived from contemporaneous diagnosis
codes.


==> sections/data.tex <==
Our data set includes records collected Stanford Hospital from 2009 through 2014.
The records were extracted the Stanford Translational Research Integrated Research Environment (STRIDE), a clinical data warehouse, where they were cleaned and de-identified before being made available for research purposes.
% We used patient data collected at Stanford Hospital from 2009 through 2014 in the Stanford Translational Research Integrated Database Environment (STRIDE).
Each patient’s data comprises a timestamped series of encounters with care providers over the five year period.
% at Stanford Hospital.
Encounters generate both structured and unstructured data.
The structured data typically consists of discrete codes from controlled vocabularies for diagnoses, medications, and procedures, along with
quantitative measurements such as vitals and laboratory measurements.
The unstructured data consists of the free text of clinical notes
written by care providers documenting each encounter and other aspects of patient care. 
In all, the warehouse contains
tens of millions of
% 49 million
encounters and
% 27 million notes
clinical notes for
%2
several million patients.
However, the effective size of the data is much smaller (roughly a million notes for a hundred thousand patients) after it
has been filtered for usable data as described below.

\subsubsection*{Text processing}
The text of the clinical notes was first processed using the National Center for Biomedical Ontology (NCBO)
Annotator \citep{lependu2013pharmacovigilance}, which
% such that each note is represented as an unordered set of terms corresponding to biomedical concepts.
% The NCBO Annotator
extracts occurrences of terms in an expansive vocabulary of biomedical
terms compiled from a collection of controlled terminologies and
biomedical ontologies.
The NCBO Annotator further flags each mention for negation
(e.g., ``atrial fibrillation was ruled out'') and family history
(e.g., ``The patient’s father had hypertension'').
Following annotation, each note is converted into a BOW representation and any terms that are not recognized as biomedical concepts are discarded.
% This is per institutional policy  and not a specific research choice.

Finally, terms are normalized to unique biomedical concepts using the Unified Medical Language System MetaThesaurus, which provides a mapping of strings to Concept Unique Identifiers (CUIs) \citep{Bodenreider2004}.
%Note that terms may be mapped to multiple concepts, and that we did
%not attempt to disambiguate between alternatives.
%Such processing may result in an improved representation, but it typically is done on a per-term basis using specialized domain knowledge and is thus beyond the scope of this work.
We retained negated concepts as distinct elements in our vocabulary because negative findings are
often informative.  We removed concepts that appeared in fewer than 50 or more than 10 million notes.  This resulted in a final vocabulary of 107,388 CUIs.  For the remainder of this paper, we will refer to CUIs as ``words'' for convenience.  
%We discuss implications of this text processing in \autoref{sec:methods} and \autoref{sec:discussion}.

%It is important to point out that the above preprocessing has several implications for our experiments and findings.
%First, the loss of word order and non-biomedical terms means that we cannot reconstruct the immediate context of each term and must instead sample context at random, as described in \autoref{sec:methods}.
%While this seems regrettable for training word embeddings, we believe that it may allow us to take advantage of a wider context, e.g., representing a medication in terms of a symptom mentioned earlier in a note.
%Further, it does not impact the BOW and topic model baselines in our experiments.

%Second, mapping terms and phrases to CUIs reduces the level of noise in the text, thereby shrinking the effective size of the vocabulary and facilitating learning.
%This may appear to run counter to the argument in favor of data-driven representations, but leveraging readily available domain knowledge seems wise.
%Further, once again, the reduction in noise favors baseline approaches more than our embedding models.

\subsubsection*{Data splits}
We evaluate our learned representations on the basis of their utility for predicting clinical events of interest occurring in the future with respect to the input clinical notes, using datasets as small as 125 patients.  Thus, in addition to the traditional split of patients into training, validation and test sets used for training, tuning of model hyper-parameters and estimation of generalization error, we also split each patient's longitudinal record into two ``eras''.  The label era comprises the last six months of each patient's record; the structured data from this era provides labels, e.g., mortality, for the target tasks.  The input era comprises the 12 months prior to the label era.  Clinical notes from this era are the inputs for both the source and target tasks.  Additionally, any labels required for source tasks are derived from the structured data in the input era.  The use of data in each of the train and test splits, along with the input and label eras, is shown in figure \ref{fig:data_use}. 

\begin{figure}[h]
\centering \includegraphics[width=0.9\textwidth]{figures/data_use_figure.jpeg}
\caption{Patient data consists of longitudinal series of records, with each record consisting of both structured (e.g., diagnosis codes) and unstructured data (clinical notes).  The source task is learned exclusively using data from the input era of the training set patients. Target tasks inputs and labels exclusively from the input and label eras of the test set patients.  Data from the label era of the training patients is unused.  The validation split used for tuning model hyperparameters for the source task is omitted for clarity.}
\label{fig:data_use}
\end{figure}

We retained only those patients with usable labels and one or more non-empty annotated clinical notes in their input era, yielding a final data set of 115,232 patients and 2,735,6487 notes.
This final set was then split into training, validation, and test sets with 69,417, 11,290, and 34,525
patients and 1,644,841, 275,684, and 815,122 notes, respectively.

==> sections/discussion.tex <==
We have presented two methods for representing clinical notes that
offer compelling advantages over BOW and topic model
representations across a range of tasks, especially with small training sets.  The
\emph{embed-and-aggregate} method in particular represents a sweet
spot in the performance-complexity trade-off because it is remarkably
simple to learn, distribute and use, requiring little in the way of specialized hardware or software. 

Our work has important limitations.  
First,the evaluation tasks are not entirely in the spirit
of the work; targets like future inpatient admissions and diagnoses are actually 
plentiful since they can be derived from structured EHR data.
It would be preferable to
evaluate on prediction targets derived from clinician chart
review for rare or subtle diagnoses, and to evaluate them in
cohorts of patients that reflect intended usage instead of the general
population.  It is for such targets that improved patient
representations can have the greatest impact.

Second, our methods start with highly
processed abstracts of the raw text.  This processing 
trades off information about the text for simplicity and ease of use.  
However, it may also leave a lot of performance on the table.  We found
that embeddings learned from randomized orderings of
the processed notes performs better in our evaluations than embeddings
learned from the full text of journal abstracts. 
In fairness, however, the latter embeddings were tuned
through intrinsic evaluations rather than prediction performance. 

Our results also beg the question of why recurrent neural net
representations, which more explicitly model the structure of the
data, do not offer a more significant performance advantage than the
embed-and-aggregate.  We suspect this is because
we do not in fact have enough data and good supervision to support
the training of a higher capacity model.  We note that the best
embed-and-aggregate representations have significantly higher
dimensionality than the best RNN representation.   
Finally, we have not addressed interpretability and portability of the
representations across institutions.
 



==> sections/experiments.tex <==
%% Figure with learning curves
% \begin{figure}[tbh]
% \subfloat[]{\includegraphics[scale=0.41,clip=true,trim=0 0 245 0]{figures/Cardiac_dysrhythmias.pdf}}
% \subfloat[\hspace{100pt}]{\includegraphics[scale=0.41]{figures/Mortality.pdf}}
% \label{fig:mortality} \\
% \subfloat[]{\includegraphics[scale=0.41,clip=true,trim=0 0 245 0]{figures/ER_visit.pdf}}
% \label{fig:er}
% \subfloat[\hspace{100pt}]{\includegraphics[scale=0.41]{figures/Inpatient_Admission.pdf}}
% \label{fig:admission}
% \caption{Target task performance as a function of training set size. (a) Cardiac dysrhythmia diagnosis. (b) Mortality.
% (c) Future ER visit. (d) Future admission.  The dimensionality of each representation is in parentheses.}
% \label{fig:results}
% \end{figure}

% \begin{figure*}[tbh]
% \subfloat[Cardiac dysrhythmias]
% {\includegraphics[scale=0.35]{figures/Cardiac_dysrhythmias.pdf}}
% \label{fig:cardiac}
% \subfloat[Mortality.]{\includegraphics[scale=0.35]{figures/Mortality.pdf}}
% \label{fig:mortality}
% \subfloat[Future ER visit.]{\includegraphics[scale=0.35]{figures/ER_visit.pdf}}
% \label{fig:er}
% \subfloat[Future admission.]{\includegraphics[scale=0.35]{figures/Inpatient_Admission.pdf}}
% \label{fig:admission}
% \caption{Caption.}
% \label{fig:results}
% \end{figure*}

Our aim is to learn effective representations of clinical notes to predict future clinical events.  Because reliable labels for clinical data are often expensive to obtain, effectiveness boils down to admitting accurate models using the representations even when the training set is quite small.  We thus designed our experiments to directly evaluate this notion of effectiveness.  Our approach uses transfer learning, in which we learn embeddings for clinical notes in a source task with abundant data and labels.  We explored two approaches to the source task.  The first approach, embed-and-aggregate, does not require any labels.  The second, recurrent neural nets, uses external labels derived from structured data (ICD-9 diagnosis codes) contemporaneous with the input notes.  Each approach effectively learns a transformation of input notes to fixed length, dense vectors summarizing the sequence of inputs.  These transformations are applied to clinical notes from the input eras of patients, and the resulting representations are used as inputs for simple linear models trained to perform new, unseen target tasks --- the prediction of 9 clinical events in the patients' label eras.  These target task models were trained on random cohorts ranging in size from 125 to 4000 patients.  The
resulting models are evaluated on held out test patients (see figure \autoref{fig:expt_setup} for an overview of the experiment).  The prediction targets include three complex outcomes --- all causes
mortality, inpatient admissions, and emergency room visits --- in
addition to the six more prevalent CCS diagnosis code categories -
cardiac dysrhythmias; diabetes mellitus without complication;
disorders of lipid metabolism; essential hypertension; spondylosis,
invertebral disc disorders, other back problems; and thyroid disorders.
Note that the former targets were not used in any source task, while
the latter targets were used in supervision of the RNN models,
although in they were contemporaneous with the inputs instead of
occurring in the future in that case.

\begin{figure}[h]
\centering \includegraphics[width=0.9\textwidth]{figures/expt_setup_figure.jpeg}
\caption{We evaluated the effectiveness of the representations learned in the source tasks by the following experiments.  We take 20 random subsamples of training patients (N = 125 through 4000) and fit an L2 regularized linear model for each of the target tasks on the subsamples.  The resulting models are evaluated on the target tasks with held out test patients on the basis of area under the receiver-operator characteristic curves.}
\label{fig:expt_setup}
\end{figure}

In order to estimate the variance due to sampling with small training sets, we take 20 random subsamples of
training patients, balanced to 20\% prevalence of positive cases, for each target task.  The
various patient representations for these subsamples are used to fit
L2 regularized logistic regression models, tuned by 5-fold cross
validation on each training subsample.
This process is repeated for N = 125, 250, 500, 1000, 2000, and 4000 random training patients.
Models fit to each subsample are evaluated on a held out test set of 34,525 patients with the natural prevalence of the outcomes.
\autoref{fig:results} and \autoref{fig:results2} show plots of performance on the three complex outcomes and one CCS code target (cardiac dysrhythmias), as function of training set size.
We include representative examples of class of representation, including baselines based on topic models and BOW.
Results for all experiments are presented in table form in Appendix \ref{app:fullresults}.

For the embed-and-aggregate representations, it was advantageous to
concatenate the min, mean and max aggregated embeddings derived from
both the clinical notes and research article abstracts.  We report
results for this representation along with the best performing
embed-and-aggregate representation using just clinical notes.  Among
the RNN representations, we found that the max aggregated GRU with 600
hidden units and random initialization generally performed best across
all tasks and subsample sizes. 
% We therefore focus on these models.

For all outcomes, we see the same general pattern: the RNN-based representation was dominant at small sample sizes ($N$ less than 1000), but for larger training sets, the embed-and-aggregate features and BOW baseline rapidly caught up and, in some cases, surpassed the RNN (ER visits for the embeddings, mortality for both).
This suggests that the difference in performance is attributable at least in part to dimensionality: the embeddings have 3-4 times as many features as the RNN, BOW another order of magnitude more.
For very small values of $N$, these high dimensional data make learning very difficult and require greater regularization.
As the number of examples approaches the number of features, (1000 examples or more), the classifier is better able to exploit the the higher dimensional representations.

For the CCS code outcomes, the RNN representation maintained a
consistent advantage over the other methods, even as the sample size
increases.
This is likely because supervision of the source task RNN models includes these outcomes, albeit contemporaneous with the inputs instead of in the future.
The source task training encourages the RNN to encode information about past diagnoses, which is unsurprisingly useful for predicting future diagnostic codes.
One could easily imagine closing the gap with the RNN by simply appending past diagnoses (or some representation thereof) to the embeddings, which already perform quite well at small values of $N$.

Both of the proposed representations dominate the topic model-based features, which have been a popular representation for clinical text in recent years \citep{halpern2012comparison,ghassemi2014unfolding,miotto2016deep}.
What is more, the topic model baseline is outperformed by the BOW baseline at even modest sample sizes (500 examples or more).
One could imagine a variety of schemes for trying to improve topic model-based performance, such as using more topics or including supervision, but previous work casts doubt on whether this will be successful \citep{halpern2012comparison}.


% not competitive on any tasks

% the complex outcomes, we found that the RNN representation
% outperforms other methods with small sample sizes (500 examples or fewer), followed closely by
% embed-and-aggregate representations.
% The RNN's advantage shrinks as sample size grows,

% We see a similar pattern with BOW, which has an order of magnitude more features: 


% Both representations dominated the topic model features, but BOW became competitive at larger sample sizes (1000 examples or more)

% outperform the baselines for all sample sizes.  However, as the sample size grows
% larger the embed-and-aggregate representations catch up to and, for
% mortality, even surpasses the RNN representation.  Furthermore, the
% embed-and-aggregate curves are steeper, suggesting that the limiting
% factor in their performance may be high dimensionality relative to the
% sample size, and that models using that representation would be best
% able to exploit larger training sample sizes. 



%The resulting models are evaluated on the test patients, which has the
%natural prevalence of the target labels.  Below we show results for
%the best performing representations of each class \textemdash a BOW
%baseline, a baseline using concatenated mean and max aggregated topic
%distributions from an LDA model with 300 topics, two
%embed-and-aggregate representations, and a recurrent neural net
%representation.

%\subsubsection*{Results with N = 500 patients}
%% In table \autoref{tab:outcomes} we report the mean Area Under the
%% Receiver-Operator Curve (AUROC) across 20 random subsamples of N = 500
%% training patients, along with the standard error of the mean, for
%% three prediction targets that are complex functions of data in the EHR
%% \textemdash mortality, inpatient admission, and er visits in the
%% future are unlikely to be straight forward mappings of input data, and
%% none of the source tasks included these outcomes as labels.

%% \begin{table}[htb]
%% \centering
%% \captionsetup{justification=centering}
%% \setlength{\tabcolsep}{6pt}
%% \begin{tabular}{lccc}
%% \toprule
%% \textbf{Representation (Dims.)}  & \multicolumn{1}{l}{\textbf{Mortality}} & \multicolumn{1}{l}{\textbf{Inpatient Admission}} & \multicolumn{1}{l}{\textbf{ER Visit}} \\
%% \midrule
%% Baseline BOW (15000) &  0.761 (0.002) & 0.701 (0.007) &  0.567 (0.01) \\
%% Baseline LDA (600) &  0.817 (0.001) & 0.746 (0.002) & 0.719 (0.002) \\
%% GloVe (1500) & 0.845 (0.002) & 0.774 (0.002)  & 0.769 (0.002) \\
%% GloVe + MCEMJ (2100) & 0.856 (0.001) & 0.778 (0.002) & 0.77 (0.001) \\
%% GRU (600) & 0.866 (0.0009) & 0.784 (0.002) & 0.767 (0.001) \\
%% \bottomrule
%% \end{tabular}
%% \caption{
%% % Evaluation on the complex outcome prediction tasks.
%% Outcome prediction performance, averaged across 20 random subsamples of N = 500 training patients. 
%% % balanced to 20\% prevalence.
%% % evaluated on the full test set.
%% % Evaluations are on the test patients using the natural prevalence of the outcomes.
%% % The dimensionality of the models are shown in parentheses.
%% }
%% \label{tab:outcomes}
%% \end{table}


%% \begin{table}[htb]
%% \centering
%% \captionsetup{justification=centering}
%% \setlength{\tabcolsep}{6pt}
%% \begin{tabular}{lccc}
%% \toprule
%% \textbf{Representation}  & \multicolumn{1}{l}{\textbf{CDYS}} & \multicolumn{1}{l}{\textbf{DM}} & \multicolumn{1}{l}{\textbf{LIPID}} \\
%% \midrule
%% Baseline BOW (15000) & 0.66 (0.008) &	0.615 (0.01) &	0.595 (0.007) \\ 
%% Baseline LDA (600) & 0.681 (0.0008)	& 0.656 (0.008) & 0.62 (0.007) \\ 
%% GloVe (1500) & 0.719 (0.002) & 0.708 (0.002) & 0.67 (0.004) \\ 
%% GloVe + MCEMJ (2100) & 0.726 (0.002)	& 0.715 (0.003)	& 0.68 (0.003) \\ 
%% GRU (600) & 0.753 (0.001)	& 0.773 (0.002)	& 0.739 (0.002) \\
%% \midrule
%%  & \multicolumn{1}{l}{\textbf{HTN}} & \multicolumn{1}{l}{\textbf{BACK}} & \multicolumn{1}{l}{\textbf{THY}} \\
%% \midrule
%% Baseline BOW (15000) &  0.63 (0.007) & 0.631 (0.01) & 0.555 (0.01) \\ 
%% Baseline LDA (600) & 0.653 (0.002) & 0.666 (0.002) & 0.601 (0.008) \\ 
%% GloVe (1500) & 0.691 (0.002) & 0.709 (0.002) & 0.668 (0.004) \\ 
%% GloVe + MCEMJ (2100) & 0.696 (0.002) & 0.714 (0.002) & 0.691 (0.003) \\ 
%% GRU (600) & 0.759 (0.002) & 0.76 (0.001) & 0.745 (0.003) \\
%% \bottomrule
%% \end{tabular}
%% \caption{
%% Diagnosis prediction performance, averaged across 20 random subsamples of N = 500 training patients. 
%% % Evaluation on the CCS code prediction tasks.  Reported
%% %   metrics are the mean and standard error of the AUROC across 20
%% %   random subsamples of training patients, balanced to 20\% prevalence.
%% %   Evaluations are on the test patients using the natural prevalence of
%% %   the outcomes.
%% CDYS = Cardiac dysrhythmias, DM =
%%   Diabetes mellitus without complication, LIPID = Disorders of lipid
%%   metabolism, HTN = Essential hypertension, BACK = Spondylosis;
%% %   invertebral disc disorders; 
%% other back problems, THY = Thyroid
%%   disorders.  }
%% \label{tab:dx}
%% \end{table}

\input{sections/intrinsic_eval}





==> sections/full_results.tex <==
\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
125 & Mortality & GRU, max pool, PubMed init (200) & 0.8401 (0.0028) \\
125 & Mortality & GRU, max pool, random init (600) & 0.8458 (0.0019) \\
125 & Mortality & GRU, max pool, random init (300) & 0.8531 (0.002) \\
125 & Mortality & GRU, max pool, PubMed init (500) & 0.8338 (0.0022) \\
125 & Mortality & Baseline - Bag of Words (15000) & 0.7243 (0.0177) \\
125 & Mortality & MCEMJ; min, mean, max pool (600) & 0.8108 (0.0038) \\
125 & Mortality & GloVe 300; min, mean, max pool (900) & 0.8041 (0.0043) \\
125 & Mortality & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.8242 (0.0019) \\
125 & Mortality & GloVe 500; min, mean, max pool (1500) & 0.8128 (0.0034) \\
125 & Mortality & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.8185 (0.0046) \\
125 & Mortality & LDA; max pool (300) & 0.7774 (0.0024) \\
125 & Mortality & LDA; max and mean pool (600) & 0.7546 (0.0137) \\
125 & Mortality & LDA; mean pool (300) & 0.7112 (0.0035) \\
125 & ER visit & GRU, max pool, PubMed init (200) & 0.7285 (0.0037) \\
125 & ER visit & GRU, max pool, random init (600) & 0.7408 (0.0039) \\
125 & ER visit & GRU, max pool, random init (300) & 0.7258 (0.0124) \\
125 & ER visit & GRU, max pool, PubMed init (500) & 0.7102 (0.0134) \\
125 & ER visit & Baseline - Bag of Words (15000) & 0.6011 (0.0144) \\
125 & ER visit & MCEMJ; min, mean, max pool (600) & 0.6884 (0.013) \\
125 & ER visit & GloVe 300; min, mean, max pool (900) & 0.7184 (0.0124) \\
125 & ER visit & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7336 (0.0065) \\
125 & ER visit & GloVe 500; min, mean, max pool (1500) & 0.7296 (0.0068) \\
125 & ER visit & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7203 (0.0065) \\
125 & ER visit & LDA; max pool (300) & 0.6396 (0.0045) \\
125 & ER visit & LDA; max and mean pool (600) & 0.6358 (0.0081) \\
125 & ER visit & LDA; mean pool (300) & 0.6068 (0.0117) \\
125 & Inpatient Admission & GRU, max pool, PubMed init (200) & 0.7496 (0.005) \\
125 & Inpatient Admission & GRU, max pool, random init (600) & 0.7326 (0.0181) \\
125 & Inpatient Admission & GRU, max pool, random init (300) & 0.7645 (0.0042) \\
125 & Inpatient Admission & GRU, max pool, PubMed init (500) & 0.7394 (0.0132) \\
125 & Inpatient Admission & Baseline - Bag of Words (15000) & 0.6298 (0.0156) \\
125 & Inpatient Admission & MCEMJ; min, mean, max pool (600) & 0.7363 (0.0026) \\
125 & Inpatient Admission & GloVe 300; min, mean, max pool (900) & 0.7434 (0.0037) \\
125 & Inpatient Admission & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7306 (0.0126) \\
125 & Inpatient Admission & GloVe 500; min, mean, max pool (1500) & 0.7409 (0.0037) \\
125 & Inpatient Admission & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7271 (0.0124) \\
125 & Inpatient Admission & LDA; max pool (300) & 0.7121 (0.0019) \\
125 & Inpatient Admission & LDA; max and mean pool (600) & 0.6984 (0.0057) \\
125 & Inpatient Admission & LDA; mean pool (300) & 0.6317 (0.0132) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
125 & Cardiac dysrhythmias & GRU, max pool, PubMed init (200) & 0.7196 (0.0028) \\
125 & Cardiac dysrhythmias & GRU, max pool, random init (600) & 0.7099 (0.0119) \\
125 & Cardiac dysrhythmias & GRU, max pool, random init (300) & 0.7301 (0.0038) \\
125 & Cardiac dysrhythmias & GRU, max pool, PubMed init (500) & 0.7239 (0.0026) \\
125 & Cardiac dysrhythmias & Baseline - Bag of Words (15000) & 0.5668 (0.0133) \\
125 & Cardiac dysrhythmias & MCEMJ; min, mean, max pool (600) & 0.6921 (0.004) \\
125 & Cardiac dysrhythmias & GloVe 300; min, mean, max pool (900) & 0.6829 (0.0037) \\
125 & Cardiac dysrhythmias & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.6844 (0.0102) \\
125 & Cardiac dysrhythmias & GloVe 500; min, mean, max pool (1500) & 0.679 (0.0074) \\
125 & Cardiac dysrhythmias & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.6884 (0.0038) \\
125 & Cardiac dysrhythmias & LDA; max pool (300) & 0.6554 (0.0097) \\
125 & Cardiac dysrhythmias & LDA; max and mean pool (600) & 0.6222 (0.0123) \\
125 & Cardiac dysrhythmias & LDA; mean pool (300) & 0.5976 (0.0078) \\
125 & Diabetes mellitus w/o complic. & GRU, max pool, PubMed init (200) & 0.7365 (0.0026) \\
125 & Diabetes mellitus w/o complic. & GRU, max pool, random init (600) & 0.7241 (0.0122) \\
125 & Diabetes mellitus w/o complic. & GRU, max pool, random init (300) & 0.74 (0.0024) \\
125 & Diabetes mellitus w/o complic. & GRU, max pool, PubMed init (500) & 0.72 (0.0052) \\
125 & Diabetes mellitus w/o complic. & Baseline - Bag of Words (15000) & 0.5747 (0.0096) \\
125 & Diabetes mellitus w/o complic. & MCEMJ; min, mean, max pool (600) & 0.6756 (0.0095) \\
125 & Diabetes mellitus w/o complic. & GloVe 300; min, mean, max pool (900) & 0.6587 (0.0083) \\
125 & Diabetes mellitus w/o complic. & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.6617 (0.0094) \\
125 & Diabetes mellitus w/o complic. & GloVe 500; min, mean, max pool (1500) & 0.6648 (0.0035) \\
125 & Diabetes mellitus w/o complic. & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.6693 (0.0046) \\
125 & Diabetes mellitus w/o complic. & LDA; max pool (300) & 0.609 (0.0142) \\
125 & Diabetes mellitus w/o complic. & LDA; max and mean pool (600) & 0.6098 (0.0109) \\
125 & Diabetes mellitus w/o complic. & LDA; mean pool (300) & 0.5638 (0.0084) \\
125 & Spondylosis (back pain) & GRU, max pool, PubMed init (200) & 0.7099 (0.0168) \\
125 & Spondylosis (back pain) & GRU, max pool, random init (600) & 0.7345 (0.0034) \\
125 & Spondylosis (back pain) & GRU, max pool, random init (300) & 0.6955 (0.0193) \\
125 & Spondylosis (back pain) & GRU, max pool, PubMed init (500) & 0.7075 (0.006) \\
125 & Spondylosis (back pain) & Baseline - Bag of Words (15000) & 0.589 (0.0095) \\
125 & Spondylosis (back pain) & MCEMJ; min, mean, max pool (600) & 0.678 (0.0042) \\
125 & Spondylosis (back pain) & GloVe 300; min, mean, max pool (900) & 0.6679 (0.0057) \\
125 & Spondylosis (back pain) & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.6602 (0.0097) \\
125 & Spondylosis (back pain) & GloVe 500; min, mean, max pool (1500) & 0.6587 (0.0091) \\
125 & Spondylosis (back pain) & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.6797 (0.0046) \\
125 & Spondylosis (back pain) & LDA; max pool (300) & 0.6073 (0.0121) \\
125 & Spondylosis (back pain) & LDA; max and mean pool (600) & 0.5632 (0.0128) \\
125 & Spondylosis (back pain) & LDA; mean pool (300) & 0.5483 (0.0061) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
125 & Disorders of lipid metabolism & GRU, max pool, PubMed init (200) & 0.6972 (0.0062) \\
125 & Disorders of lipid metabolism & GRU, max pool, random init (600) & 0.7089 (0.0033) \\
125 & Disorders of lipid metabolism & GRU, max pool, random init (300) & 0.6944 (0.0151) \\
125 & Disorders of lipid metabolism & GRU, max pool, PubMed init (500) & 0.697 (0.0026) \\
125 & Disorders of lipid metabolism & Baseline - Bag of Words (15000) & 0.5598 (0.0071) \\
125 & Disorders of lipid metabolism & MCEMJ; min, mean, max pool (600) & 0.6197 (0.0077) \\
125 & Disorders of lipid metabolism & GloVe 300; min, mean, max pool (900) & 0.6011 (0.0124) \\
125 & Disorders of lipid metabolism & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.6243 (0.0086) \\
125 & Disorders of lipid metabolism & GloVe 500; min, mean, max pool (1500) & 0.6259 (0.007) \\
125 & Disorders of lipid metabolism & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.6224 (0.0103) \\
125 & Disorders of lipid metabolism & LDA; max pool (300) & 0.571 (0.0104) \\
125 & Disorders of lipid metabolism & LDA; max and mean pool (600) & 0.5839 (0.0063) \\
125 & Disorders of lipid metabolism & LDA; mean pool (300) & 0.5392 (0.0061) \\
125 & Essential hypertension & GRU, max pool, PubMed init (200) & 0.7173 (0.0116) \\
125 & Essential hypertension & GRU, max pool, random init (600) & 0.7076 (0.0114) \\
125 & Essential hypertension & GRU, max pool, random init (300) & 0.7324 (0.0025) \\
125 & Essential hypertension & GRU, max pool, PubMed init (500) & 0.7162 (0.003) \\
125 & Essential hypertension & Baseline - Bag of Words (15000) & 0.5563 (0.0071) \\
125 & Essential hypertension & MCEMJ; min, mean, max pool (600) & 0.6444 (0.0115) \\
125 & Essential hypertension & GloVe 300; min, mean, max pool (900) & 0.6452 (0.0083) \\
125 & Essential hypertension & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.6499 (0.0087) \\
125 & Essential hypertension & GloVe 500; min, mean, max pool (1500) & 0.6443 (0.0069) \\
125 & Essential hypertension & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.6409 (0.0118) \\
125 & Essential hypertension & LDA; max pool (300) & 0.6206 (0.0073) \\
125 & Essential hypertension & LDA; max and mean pool (600) & 0.5951 (0.0095) \\
125 & Essential hypertension & LDA; mean pool (300) & 0.5514 (0.0059) \\
125 & Thyroid disorders & GRU, max pool, PubMed init (200) & 0.6574 (0.0094) \\
125 & Thyroid disorders & GRU, max pool, random init (600) & 0.6902 (0.0151) \\
125 & Thyroid disorders & GRU, max pool, random init (300) & 0.6907 (0.0057) \\
125 & Thyroid disorders & GRU, max pool, PubMed init (500) & 0.6452 (0.0052) \\
125 & Thyroid disorders & Baseline - Bag of Words (15000) & 0.5346 (0.0055) \\
125 & Thyroid disorders & MCEMJ; min, mean, max pool (600) & 0.6388 (0.0054) \\
125 & Thyroid disorders & GloVe 300; min, mean, max pool (900) & 0.6141 (0.0063) \\
125 & Thyroid disorders & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.6238 (0.008) \\
125 & Thyroid disorders & GloVe 500; min, mean, max pool (1500) & 0.6124 (0.0096) \\
125 & Thyroid disorders & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.6265 (0.0079) \\
125 & Thyroid disorders & LDA; max pool (300) & 0.5737 (0.0077) \\
125 & Thyroid disorders & LDA; max and mean pool (600) & 0.553 (0.0079) \\
125 & Thyroid disorders & LDA; mean pool (300) & 0.525 (0.0054) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
250 & Mortality & GRU, max pool, PubMed init (200) & 0.849 (0.0012) \\
250 & Mortality & GRU, max pool, random init (600) & 0.8577 (0.0013) \\
250 & Mortality & GRU, max pool, random init (300) & 0.8628 (0.001) \\
250 & Mortality & GRU, max pool, PubMed init (500) & 0.8429 (0.0014) \\
250 & Mortality & Baseline - Bag of Words (15000) & 0.7959 (0.0157) \\
250 & Mortality & MCEMJ; min, mean, max pool (600) & 0.8241 (0.0014) \\
250 & Mortality & GloVe 300; min, mean, max pool (900) & 0.8278 (0.0025) \\
250 & Mortality & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.8379 (0.0021) \\
250 & Mortality & GloVe 500; min, mean, max pool (1500) & 0.8317 (0.0016) \\
250 & Mortality & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.8443 (0.0022) \\
250 & Mortality & LDA; max pool (300) & 0.8008 (0.0019) \\
250 & Mortality & LDA; max and mean pool (600) & 0.7972 (0.0024) \\
250 & Mortality & LDA; mean pool (300) & 0.7359 (0.0127) \\
250 & ER visit & GRU, max pool, PubMed init (200) & 0.7487 (0.0028) \\
250 & ER visit & GRU, max pool, random init (600) & 0.7556 (0.0022) \\
250 & ER visit & GRU, max pool, random init (300) & 0.7452 (0.0024) \\
250 & ER visit & GRU, max pool, PubMed init (500) & 0.7447 (0.0036) \\
250 & ER visit & Baseline - Bag of Words (15000) & 0.7038 (0.0113) \\
250 & ER visit & MCEMJ; min, mean, max pool (600) & 0.7426 (0.0028) \\
250 & ER visit & GloVe 300; min, mean, max pool (900) & 0.7446 (0.0069) \\
250 & ER visit & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7593 (0.0028) \\
250 & ER visit & GloVe 500; min, mean, max pool (1500) & 0.7433 (0.0046) \\
250 & ER visit & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7538 (0.0024) \\
250 & ER visit & LDA; max pool (300) & 0.6591 (0.0093) \\
250 & ER visit & LDA; max and mean pool (600) & 0.6545 (0.0126) \\
250 & ER visit & LDA; mean pool (300) & 0.6516 (0.0089) \\
250 & Inpatient Admission & GRU, max pool, PubMed init (200) & 0.7631 (0.0042) \\
250 & Inpatient Admission & GRU, max pool, random init (600) & 0.7702 (0.0029) \\
250 & Inpatient Admission & GRU, max pool, random init (300) & 0.7832 (0.002) \\
250 & Inpatient Admission & GRU, max pool, PubMed init (500) & 0.7641 (0.0025) \\
250 & Inpatient Admission & Baseline - Bag of Words (15000) & 0.708 (0.016) \\
250 & Inpatient Admission & MCEMJ; min, mean, max pool (600) & 0.7504 (0.0028) \\
250 & Inpatient Admission & GloVe 300; min, mean, max pool (900) & 0.7613 (0.003) \\
250 & Inpatient Admission & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7572 (0.0044) \\
250 & Inpatient Admission & GloVe 500; min, mean, max pool (1500) & 0.7594 (0.0038) \\
250 & Inpatient Admission & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7544 (0.0036) \\
250 & Inpatient Admission & LDA; max pool (300) & 0.7287 (0.0022) \\
250 & Inpatient Admission & LDA; max and mean pool (600) & 0.7249 (0.0031) \\
250 & Inpatient Admission & LDA; mean pool (300) & 0.6865 (0.0025) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
250 & Cardiac dysrhythmias & GRU, max pool, PubMed init (200) & 0.7267 (0.0026) \\
250 & Cardiac dysrhythmias & GRU, max pool, random init (600) & 0.7418 (0.0019) \\
250 & Cardiac dysrhythmias & GRU, max pool, random init (300) & 0.7434 (0.0019) \\
250 & Cardiac dysrhythmias & GRU, max pool, PubMed init (500) & 0.7238 (0.0018) \\
250 & Cardiac dysrhythmias & Baseline - Bag of Words (15000) & 0.6511 (0.012) \\
250 & Cardiac dysrhythmias & MCEMJ; min, mean, max pool (600) & 0.707 (0.0032) \\
250 & Cardiac dysrhythmias & GloVe 300; min, mean, max pool (900) & 0.7052 (0.0025) \\
250 & Cardiac dysrhythmias & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7 (0.0109) \\
250 & Cardiac dysrhythmias & GloVe 500; min, mean, max pool (1500) & 0.6989 (0.0032) \\
250 & Cardiac dysrhythmias & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7067 (0.0027) \\
250 & Cardiac dysrhythmias & LDA; max pool (300) & 0.6762 (0.0014) \\
250 & Cardiac dysrhythmias & LDA; max and mean pool (600) & 0.6693 (0.0014) \\
250 & Cardiac dysrhythmias & LDA; mean pool (300) & 0.6286 (0.0022) \\
250 & Diabetes mellitus w/o complic. & GRU, max pool, PubMed init (200) & 0.7437 (0.0047) \\
250 & Diabetes mellitus w/o complic. & GRU, max pool, random init (600) & 0.7579 (0.0024) \\
250 & Diabetes mellitus w/o complic. & GRU, max pool, random init (300) & 0.7541 (0.0017) \\
250 & Diabetes mellitus w/o complic. & GRU, max pool, PubMed init (500) & 0.7393 (0.0022) \\
250 & Diabetes mellitus w/o complic. & Baseline - Bag of Words (15000) & 0.6135 (0.0133) \\
250 & Diabetes mellitus w/o complic. & MCEMJ; min, mean, max pool (600) & 0.696 (0.0029) \\
250 & Diabetes mellitus w/o complic. & GloVe 300; min, mean, max pool (900) & 0.6775 (0.0047) \\
250 & Diabetes mellitus w/o complic. & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.6905 (0.004) \\
250 & Diabetes mellitus w/o complic. & GloVe 500; min, mean, max pool (1500) & 0.6776 (0.0098) \\
250 & Diabetes mellitus w/o complic. & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.6887 (0.004) \\
250 & Diabetes mellitus w/o complic. & LDA; max pool (300) & 0.6584 (0.0016) \\
250 & Diabetes mellitus w/o complic. & LDA; max and mean pool (600) & 0.6431 (0.0078) \\
250 & Diabetes mellitus w/o complic. & LDA; mean pool (300) & 0.5694 (0.0086) \\
250 & Spondylosis (back pain) & GRU, max pool, PubMed init (200) & 0.7396 (0.0028) \\
250 & Spondylosis (back pain) & GRU, max pool, random init (600) & 0.7462 (0.0029) \\
250 & Spondylosis (back pain) & GRU, max pool, random init (300) & 0.7426 (0.0028) \\
250 & Spondylosis (back pain) & GRU, max pool, PubMed init (500) & 0.7264 (0.0027) \\
250 & Spondylosis (back pain) & Baseline - Bag of Words (15000) & 0.651 (0.0035) \\
250 & Spondylosis (back pain) & MCEMJ; min, mean, max pool (600) & 0.6862 (0.0034) \\
250 & Spondylosis (back pain) & GloVe 300; min, mean, max pool (900) & 0.6838 (0.0036) \\
250 & Spondylosis (back pain) & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.6811 (0.0102) \\
250 & Spondylosis (back pain) & GloVe 500; min, mean, max pool (1500) & 0.6897 (0.0043) \\
250 & Spondylosis (back pain) & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.6969 (0.0036) \\
250 & Spondylosis (back pain) & LDA; max pool (300) & 0.6475 (0.0036) \\
250 & Spondylosis (back pain) & LDA; max and mean pool (600) & 0.6367 (0.0075) \\
250 & Spondylosis (back pain) & LDA; mean pool (300) & 0.5649 (0.008) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
250 & Disorders of lipid metabolism & GRU, max pool, PubMed init (200) & 0.714 (0.0021) \\
250 & Disorders of lipid metabolism & GRU, max pool, random init (600) & 0.7204 (0.0033) \\
250 & Disorders of lipid metabolism & GRU, max pool, random init (300) & 0.7212 (0.0027) \\
250 & Disorders of lipid metabolism & GRU, max pool, PubMed init (500) & 0.7099 (0.0023) \\
250 & Disorders of lipid metabolism & Baseline - Bag of Words (15000) & 0.6057 (0.0042) \\
250 & Disorders of lipid metabolism & MCEMJ; min, mean, max pool (600) & 0.6522 (0.0038) \\
250 & Disorders of lipid metabolism & GloVe 300; min, mean, max pool (900) & 0.6506 (0.006) \\
250 & Disorders of lipid metabolism & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.6505 (0.0047) \\
250 & Disorders of lipid metabolism & GloVe 500; min, mean, max pool (1500) & 0.6555 (0.0045) \\
250 & Disorders of lipid metabolism & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.6576 (0.0044) \\
250 & Disorders of lipid metabolism & LDA; max pool (300) & 0.604 (0.0075) \\
250 & Disorders of lipid metabolism & LDA; max and mean pool (600) & 0.5942 (0.0092) \\
250 & Disorders of lipid metabolism & LDA; mean pool (300) & 0.5618 (0.0043) \\
250 & Essential hypertension & GRU, max pool, PubMed init (200) & 0.7373 (0.0023) \\
250 & Essential hypertension & GRU, max pool, random init (600) & 0.7399 (0.003) \\
250 & Essential hypertension & GRU, max pool, random init (300) & 0.7413 (0.0027) \\
250 & Essential hypertension & GRU, max pool, PubMed init (500) & 0.731 (0.0028) \\
250 & Essential hypertension & Baseline - Bag of Words (15000) & 0.5942 (0.0113) \\
250 & Essential hypertension & MCEMJ; min, mean, max pool (600) & 0.6749 (0.0027) \\
250 & Essential hypertension & GloVe 300; min, mean, max pool (900) & 0.668 (0.0031) \\
250 & Essential hypertension & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.6726 (0.0037) \\
250 & Essential hypertension & GloVe 500; min, mean, max pool (1500) & 0.6629 (0.0092) \\
250 & Essential hypertension & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.6776 (0.0037) \\
250 & Essential hypertension & LDA; max pool (300) & 0.6378 (0.0075) \\
250 & Essential hypertension & LDA; max and mean pool (600) & 0.6173 (0.0097) \\
250 & Essential hypertension & LDA; mean pool (300) & 0.5715 (0.0074) \\
250 & Thyroid disorders & GRU, max pool, PubMed init (200) & 0.682 (0.0048) \\
250 & Thyroid disorders & GRU, max pool, random init (600) & 0.7261 (0.003) \\
250 & Thyroid disorders & GRU, max pool, random init (300) & 0.7215 (0.0027) \\
250 & Thyroid disorders & GRU, max pool, PubMed init (500) & 0.6602 (0.0038) \\
250 & Thyroid disorders & Baseline - Bag of Words (15000) & 0.5773 (0.0092) \\
250 & Thyroid disorders & MCEMJ; min, mean, max pool (600) & 0.6631 (0.0092) \\
250 & Thyroid disorders & GloVe 300; min, mean, max pool (900) & 0.6421 (0.004) \\
250 & Thyroid disorders & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.6511 (0.0092) \\
250 & Thyroid disorders & GloVe 500; min, mean, max pool (1500) & 0.6506 (0.0047) \\
250 & Thyroid disorders & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.6584 (0.0038) \\
250 & Thyroid disorders & LDA; max pool (300) & 0.6048 (0.0012) \\
250 & Thyroid disorders & LDA; max and mean pool (600) & 0.5802 (0.0078) \\
250 & Thyroid disorders & LDA; mean pool (300) & 0.5415 (0.004) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
500 & Mortality & GRU, max pool, PubMed init (200) & 0.8534 (0.0009) \\
500 & Mortality & GRU, max pool, random init (600) & 0.8659 (0.0009) \\
500 & Mortality & GRU, max pool, random init (300) & 0.866 (0.0007) \\
500 & Mortality & GRU, max pool, PubMed init (500) & 0.8493 (0.0008) \\
500 & Mortality & Baseline - Bag of Words (15000) & 0.851 (0.0013) \\
500 & Mortality & MCEMJ; min, mean, max pool (600) & 0.8273 (0.0018) \\
500 & Mortality & GloVe 300; min, mean, max pool (900) & 0.8336 (0.0018) \\
500 & Mortality & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.8521 (0.0017) \\
500 & Mortality & GloVe 500; min, mean, max pool (1500) & 0.845 (0.0015) \\
500 & Mortality & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.8556 (0.0014) \\
500 & Mortality & LDA; max pool (300) & 0.8261 (0.0019) \\
500 & Mortality & LDA; max and mean pool (600) & 0.8169 (0.0014) \\
500 & Mortality & LDA; mean pool (300) & 0.7711 (0.0024) \\
500 & ER visit & GRU, max pool, PubMed init (200) & 0.7577 (0.0016) \\
500 & ER visit & GRU, max pool, random init (600) & 0.7669 (0.0012) \\
500 & ER visit & GRU, max pool, random init (300) & 0.7565 (0.0024) \\
500 & ER visit & GRU, max pool, PubMed init (500) & 0.76 (0.0014) \\
500 & ER visit & Baseline - Bag of Words (15000) & 0.7401 (0.0127) \\
500 & ER visit & MCEMJ; min, mean, max pool (600) & 0.7588 (0.0027) \\
500 & ER visit & GloVe 300; min, mean, max pool (900) & 0.7676 (0.0012) \\
500 & ER visit & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.771 (0.0013) \\
500 & ER visit & GloVe 500; min, mean, max pool (1500) & 0.7692 (0.0015) \\
500 & ER visit & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7704 (0.0014) \\
500 & ER visit & LDA; max pool (300) & 0.6982 (0.0034) \\
500 & ER visit & LDA; max and mean pool (600) & 0.719 (0.0016) \\
500 & ER visit & LDA; mean pool (300) & 0.6942 (0.0024) \\
500 & Inpatient Admission & GRU, max pool, PubMed init (200) & 0.7786 (0.0021) \\
500 & Inpatient Admission & GRU, max pool, random init (600) & 0.7836 (0.0021) \\
500 & Inpatient Admission & GRU, max pool, random init (300) & 0.7878 (0.002) \\
500 & Inpatient Admission & GRU, max pool, PubMed init (500) & 0.7757 (0.0013) \\
500 & Inpatient Admission & Baseline - Bag of Words (15000) & 0.7608 (0.0015) \\
500 & Inpatient Admission & MCEMJ; min, mean, max pool (600) & 0.7632 (0.0016) \\
500 & Inpatient Admission & GloVe 300; min, mean, max pool (900) & 0.7695 (0.0021) \\
500 & Inpatient Admission & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7774 (0.002) \\
500 & Inpatient Admission & GloVe 500; min, mean, max pool (1500) & 0.7744 (0.0017) \\
500 & Inpatient Admission & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7782 (0.0017) \\
500 & Inpatient Admission & LDA; max pool (300) & 0.7423 (0.0027) \\
500 & Inpatient Admission & LDA; max and mean pool (600) & 0.7459 (0.0015) \\
500 & Inpatient Admission & LDA; mean pool (300) & 0.7126 (0.0024) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
500 & Cardiac dysrhythmias & GRU, max pool, PubMed init (200) & 0.7336 (0.0025) \\
500 & Cardiac dysrhythmias & GRU, max pool, random init (600) & 0.7526 (0.0013) \\
500 & Cardiac dysrhythmias & GRU, max pool, random init (300) & 0.7493 (0.0014) \\
500 & Cardiac dysrhythmias & GRU, max pool, PubMed init (500) & 0.737 (0.0011) \\
500 & Cardiac dysrhythmias & Baseline - Bag of Words (15000) & 0.6797 (0.0138) \\
500 & Cardiac dysrhythmias & MCEMJ; min, mean, max pool (600) & 0.7215 (0.0023) \\
500 & Cardiac dysrhythmias & GloVe 300; min, mean, max pool (900) & 0.7184 (0.0028) \\
500 & Cardiac dysrhythmias & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7272 (0.0023) \\
500 & Cardiac dysrhythmias & GloVe 500; min, mean, max pool (1500) & 0.719 (0.0022) \\
500 & Cardiac dysrhythmias & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.726 (0.0019) \\
500 & Cardiac dysrhythmias & LDA; max pool (300) & 0.6819 (0.0012) \\
500 & Cardiac dysrhythmias & LDA; max and mean pool (600) & 0.6808 (0.0008) \\
500 & Cardiac dysrhythmias & LDA; mean pool (300) & 0.6422 (0.001) \\
500 & Diabetes mellitus w/o complic. & GRU, max pool, PubMed init (200) & 0.7557 (0.0014) \\
500 & Diabetes mellitus w/o complic. & GRU, max pool, random init (600) & 0.773 (0.002) \\
500 & Diabetes mellitus w/o complic. & GRU, max pool, random init (300) & 0.764 (0.0013) \\
500 & Diabetes mellitus w/o complic. & GRU, max pool, PubMed init (500) & 0.7537 (0.0018) \\
500 & Diabetes mellitus w/o complic. & Baseline - Bag of Words (15000) & 0.6697 (0.0133) \\
500 & Diabetes mellitus w/o complic. & MCEMJ; min, mean, max pool (600) & 0.7094 (0.0015) \\
500 & Diabetes mellitus w/o complic. & GloVe 300; min, mean, max pool (900) & 0.7049 (0.0026) \\
500 & Diabetes mellitus w/o complic. & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7119 (0.0025) \\
500 & Diabetes mellitus w/o complic. & GloVe 500; min, mean, max pool (1500) & 0.7081 (0.0022) \\
500 & Diabetes mellitus w/o complic. & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7152 (0.003) \\
500 & Diabetes mellitus w/o complic. & LDA; max pool (300) & 0.6677 (0.0014) \\
500 & Diabetes mellitus w/o complic. & LDA; max and mean pool (600) & 0.6561 (0.0085) \\
500 & Diabetes mellitus w/o complic. & LDA; mean pool (300) & 0.5949 (0.0098) \\
500 & Spondylosis (back pain) & GRU, max pool, PubMed init (200) & 0.7481 (0.002) \\
500 & Spondylosis (back pain) & GRU, max pool, random init (600) & 0.76 (0.0011) \\
500 & Spondylosis (back pain) & GRU, max pool, random init (300) & 0.7523 (0.0019) \\
500 & Spondylosis (back pain) & GRU, max pool, PubMed init (500) & 0.739 (0.0011) \\
500 & Spondylosis (back pain) & Baseline - Bag of Words (15000) & 0.6713 (0.0132) \\
500 & Spondylosis (back pain) & MCEMJ; min, mean, max pool (600) & 0.7052 (0.0019) \\
500 & Spondylosis (back pain) & GloVe 300; min, mean, max pool (900) & 0.7002 (0.0029) \\
500 & Spondylosis (back pain) & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7078 (0.0035) \\
500 & Spondylosis (back pain) & GloVe 500; min, mean, max pool (1500) & 0.7086 (0.0021) \\
500 & Spondylosis (back pain) & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7137 (0.0021) \\
500 & Spondylosis (back pain) & LDA; max pool (300) & 0.6686 (0.0018) \\
500 & Spondylosis (back pain) & LDA; max and mean pool (600) & 0.6655 (0.0015) \\
500 & Spondylosis (back pain) & LDA; mean pool (300) & 0.6046 (0.0038) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
500 & Disorders of lipid metabolism & GRU, max pool, PubMed init (200) & 0.7284 (0.002) \\
500 & Disorders of lipid metabolism & GRU, max pool, random init (600) & 0.7389 (0.0016) \\
500 & Disorders of lipid metabolism & GRU, max pool, random init (300) & 0.739 (0.0013) \\
500 & Disorders of lipid metabolism & GRU, max pool, PubMed init (500) & 0.7275 (0.0017) \\
500 & Disorders of lipid metabolism & Baseline - Bag of Words (15000) & 0.6276 (0.0126) \\
500 & Disorders of lipid metabolism & MCEMJ; min, mean, max pool (600) & 0.6631 (0.0039) \\
500 & Disorders of lipid metabolism & GloVe 300; min, mean, max pool (900) & 0.6664 (0.0032) \\
500 & Disorders of lipid metabolism & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.6728 (0.0038) \\
500 & Disorders of lipid metabolism & GloVe 500; min, mean, max pool (1500) & 0.6698 (0.004) \\
500 & Disorders of lipid metabolism & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.68 (0.0026) \\
500 & Disorders of lipid metabolism & LDA; max pool (300) & 0.6233 (0.0034) \\
500 & Disorders of lipid metabolism & LDA; max and mean pool (600) & 0.6199 (0.0066) \\
500 & Disorders of lipid metabolism & LDA; mean pool (300) & 0.5779 (0.0051) \\
500 & Essential hypertension & GRU, max pool, PubMed init (200) & 0.7517 (0.0031) \\
500 & Essential hypertension & GRU, max pool, random init (600) & 0.7592 (0.0019) \\
500 & Essential hypertension & GRU, max pool, random init (300) & 0.7547 (0.0022) \\
500 & Essential hypertension & GRU, max pool, PubMed init (500) & 0.7479 (0.0016) \\
500 & Essential hypertension & Baseline - Bag of Words (15000) & 0.66 (0.0019) \\
500 & Essential hypertension & MCEMJ; min, mean, max pool (600) & 0.6893 (0.0021) \\
500 & Essential hypertension & GloVe 300; min, mean, max pool (900) & 0.692 (0.0021) \\
500 & Essential hypertension & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.6967 (0.0021) \\
500 & Essential hypertension & GloVe 500; min, mean, max pool (1500) & 0.6911 (0.0022) \\
500 & Essential hypertension & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.6958 (0.0024) \\
500 & Essential hypertension & LDA; max pool (300) & 0.6456 (0.0082) \\
500 & Essential hypertension & LDA; max and mean pool (600) & 0.6533 (0.002) \\
500 & Essential hypertension & LDA; mean pool (300) & 0.575 (0.0094) \\
500 & Thyroid disorders & GRU, max pool, PubMed init (200) & 0.7046 (0.0019) \\
500 & Thyroid disorders & GRU, max pool, random init (600) & 0.7447 (0.0028) \\
500 & Thyroid disorders & GRU, max pool, random init (300) & 0.7344 (0.003) \\
500 & Thyroid disorders & GRU, max pool, PubMed init (500) & 0.6779 (0.0024) \\
500 & Thyroid disorders & Baseline - Bag of Words (15000) & 0.6319 (0.002) \\
500 & Thyroid disorders & MCEMJ; min, mean, max pool (600) & 0.6958 (0.0023) \\
500 & Thyroid disorders & GloVe 300; min, mean, max pool (900) & 0.6663 (0.0019) \\
500 & Thyroid disorders & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.6923 (0.0032) \\
500 & Thyroid disorders & GloVe 500; min, mean, max pool (1500) & 0.6685 (0.0043) \\
500 & Thyroid disorders & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.6914 (0.003) \\
500 & Thyroid disorders & LDA; max pool (300) & 0.6128 (0.0015) \\
500 & Thyroid disorders & LDA; max and mean pool (600) & 0.6011 (0.008) \\
500 & Thyroid disorders & LDA; mean pool (300) & 0.544 (0.0063) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
1000 & Mortality & GRU, max pool, PubMed init (200) & 0.8588 (0.0007) \\
1000 & Mortality & GRU, max pool, random init (600) & 0.8735 (0.0007) \\
1000 & Mortality & GRU, max pool, random init (300) & 0.8728 (0.0005) \\
1000 & Mortality & GRU, max pool, PubMed init (500) & 0.8566 (0.0008) \\
1000 & Mortality & Baseline - Bag of Words (15000) & 0.8777 (0.0006) \\
1000 & Mortality & MCEMJ; min, mean, max pool (600) & 0.8641 (0.0012) \\
1000 & Mortality & GloVe 300; min, mean, max pool (900) & 0.8408 (0.0015) \\
1000 & Mortality & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.8578 (0.0014) \\
1000 & Mortality & GloVe 500; min, mean, max pool (1500) & 0.8532 (0.0012) \\
1000 & Mortality & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.8632 (0.0011) \\
1000 & Mortality & LDA; max pool (300) & 0.8432 (0.0013) \\
1000 & Mortality & LDA; max and mean pool (600) & 0.8382 (0.0013) \\
1000 & Mortality & LDA; mean pool (300) & 0.7933 (0.0015) \\
1000 & ER visit & GRU, max pool, PubMed init (200) & 0.7663 (0.001) \\
1000 & ER visit & GRU, max pool, random init (600) & 0.7763 (0.0009) \\
1000 & ER visit & GRU, max pool, random init (300) & 0.7678 (0.0009) \\
1000 & ER visit & GRU, max pool, PubMed init (500) & 0.7649 (0.0011) \\
1000 & ER visit & Baseline - Bag of Words (15000) & 0.7678 (0.0009) \\
1000 & ER visit & MCEMJ; min, mean, max pool (600) & 0.7719 (0.0014) \\
1000 & ER visit & GloVe 300; min, mean, max pool (900) & 0.7765 (0.0007) \\
1000 & ER visit & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7793 (0.0008) \\
1000 & ER visit & GloVe 500; min, mean, max pool (1500) & 0.7783 (0.0008) \\
1000 & ER visit & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7803 (0.001) \\
1000 & ER visit & LDA; max pool (300) & 0.7211 (0.0015) \\
1000 & ER visit & LDA; max and mean pool (600) & 0.7336 (0.0015) \\
1000 & ER visit & LDA; mean pool (300) & 0.7148 (0.002) \\
1000 & Inpatient Admission & GRU, max pool, PubMed init (200) & 0.7896 (0.0009) \\
1000 & Inpatient Admission & GRU, max pool, random init (600) & 0.7945 (0.0008) \\
1000 & Inpatient Admission & GRU, max pool, random init (300) & 0.7952 (0.0009) \\
1000 & Inpatient Admission & GRU, max pool, PubMed init (500) & 0.7831 (0.0008) \\
1000 & Inpatient Admission & Baseline - Bag of Words (15000) & 0.7812 (0.0008) \\
1000 & Inpatient Admission & MCEMJ; min, mean, max pool (600) & 0.7804 (0.0014) \\
1000 & Inpatient Admission & GloVe 300; min, mean, max pool (900) & 0.7798 (0.0012) \\
1000 & Inpatient Admission & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7854 (0.0009) \\
1000 & Inpatient Admission & GloVe 500; min, mean, max pool (1500) & 0.7838 (0.0011) \\
1000 & Inpatient Admission & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7874 (0.0015) \\
1000 & Inpatient Admission & LDA; max pool (300) & 0.7589 (0.0017) \\
1000 & Inpatient Admission & LDA; max and mean pool (600) & 0.7603 (0.0016) \\
1000 & Inpatient Admission & LDA; mean pool (300) & 0.7338 (0.0016) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
1000 & Cardiac dysrhythmias & GRU, max pool, PubMed init (200) & 0.7435 (0.0012) \\
1000 & Cardiac dysrhythmias & GRU, max pool, random init (600) & 0.7574 (0.0009) \\
1000 & Cardiac dysrhythmias & GRU, max pool, random init (300) & 0.7549 (0.001) \\
1000 & Cardiac dysrhythmias & GRU, max pool, PubMed init (500) & 0.7425 (0.002) \\
1000 & Cardiac dysrhythmias & Baseline - Bag of Words (15000) & 0.7272 (0.001) \\
1000 & Cardiac dysrhythmias & MCEMJ; min, mean, max pool (600) & 0.7401 (0.001) \\
1000 & Cardiac dysrhythmias & GloVe 300; min, mean, max pool (900) & 0.7325 (0.0011) \\
1000 & Cardiac dysrhythmias & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7394 (0.0016) \\
1000 & Cardiac dysrhythmias & GloVe 500; min, mean, max pool (1500) & 0.7338 (0.001) \\
1000 & Cardiac dysrhythmias & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7408 (0.0012) \\
1000 & Cardiac dysrhythmias & LDA; max pool (300) & 0.6941 (0.0016) \\
1000 & Cardiac dysrhythmias & LDA; max and mean pool (600) & 0.6923 (0.0015) \\
1000 & Cardiac dysrhythmias & LDA; mean pool (300) & 0.6587 (0.0017) \\
1000 & Diabetes mellitus w/o complic. & GRU, max pool, PubMed init (200) & 0.7645 (0.0015) \\
1000 & Diabetes mellitus w/o complic. & GRU, max pool, random init (600) & 0.7885 (0.0009) \\
1000 & Diabetes mellitus w/o complic. & GRU, max pool, random init (300) & 0.7734 (0.0013) \\
1000 & Diabetes mellitus w/o complic. & GRU, max pool, PubMed init (500) & 0.7587 (0.0012) \\
1000 & Diabetes mellitus w/o complic. & Baseline - Bag of Words (15000) & 0.7226 (0.0018) \\
1000 & Diabetes mellitus w/o complic. & MCEMJ; min, mean, max pool (600) & 0.7384 (0.0018) \\
1000 & Diabetes mellitus w/o complic. & GloVe 300; min, mean, max pool (900) & 0.7169 (0.0015) \\
1000 & Diabetes mellitus w/o complic. & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7341 (0.0018) \\
1000 & Diabetes mellitus w/o complic. & GloVe 500; min, mean, max pool (1500) & 0.7256 (0.0019) \\
1000 & Diabetes mellitus w/o complic. & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7384 (0.0019) \\
1000 & Diabetes mellitus w/o complic. & LDA; max pool (300) & 0.6806 (0.0018) \\
1000 & Diabetes mellitus w/o complic. & LDA; max and mean pool (600) & 0.6834 (0.0018) \\
1000 & Diabetes mellitus w/o complic. & LDA; mean pool (300) & 0.6325 (0.0019) \\
1000 & Spondylosis (back pain) & GRU, max pool, PubMed init (200) & 0.7556 (0.0013) \\
1000 & Spondylosis (back pain) & GRU, max pool, random init (600) & 0.7667 (0.0009) \\
1000 & Spondylosis (back pain) & GRU, max pool, random init (300) & 0.7599 (0.0009) \\
1000 & Spondylosis (back pain) & GRU, max pool, PubMed init (500) & 0.7469 (0.0011) \\
1000 & Spondylosis (back pain) & Baseline - Bag of Words (15000) & 0.7115 (0.0016) \\
1000 & Spondylosis (back pain) & MCEMJ; min, mean, max pool (600) & 0.7252 (0.001) \\
1000 & Spondylosis (back pain) & GloVe 300; min, mean, max pool (900) & 0.7178 (0.0015) \\
1000 & Spondylosis (back pain) & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.729 (0.0012) \\
1000 & Spondylosis (back pain) & GloVe 500; min, mean, max pool (1500) & 0.7229 (0.0015) \\
1000 & Spondylosis (back pain) & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7283 (0.0016) \\
1000 & Spondylosis (back pain) & LDA; max pool (300) & 0.6802 (0.0018) \\
1000 & Spondylosis (back pain) & LDA; max and mean pool (600) & 0.6827 (0.0017) \\
1000 & Spondylosis (back pain) & LDA; mean pool (300) & 0.6281 (0.0025) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
1000 & Disorders of lipid metabolism & GRU, max pool, PubMed init (200) & 0.7443 (0.0015) \\
1000 & Disorders of lipid metabolism & GRU, max pool, random init (600) & 0.7509 (0.0011) \\
1000 & Disorders of lipid metabolism & GRU, max pool, random init (300) & 0.7481 (0.0013) \\
1000 & Disorders of lipid metabolism & GRU, max pool, PubMed init (500) & 0.7331 (0.0016) \\
1000 & Disorders of lipid metabolism & Baseline - Bag of Words (15000) & 0.6787 (0.0022) \\
1000 & Disorders of lipid metabolism & MCEMJ; min, mean, max pool (600) & 0.6954 (0.0016) \\
1000 & Disorders of lipid metabolism & GloVe 300; min, mean, max pool (900) & 0.6905 (0.0018) \\
1000 & Disorders of lipid metabolism & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.6989 (0.0017) \\
1000 & Disorders of lipid metabolism & GloVe 500; min, mean, max pool (1500) & 0.6904 (0.0023) \\
1000 & Disorders of lipid metabolism & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7014 (0.0019) \\
1000 & Disorders of lipid metabolism & LDA; max pool (300) & 0.6375 (0.002) \\
1000 & Disorders of lipid metabolism & LDA; max and mean pool (600) & 0.6442 (0.002) \\
1000 & Disorders of lipid metabolism & LDA; mean pool (300) & 0.6001 (0.0056) \\
1000 & Essential hypertension & GRU, max pool, PubMed init (200) & 0.7659 (0.001) \\
1000 & Essential hypertension & GRU, max pool, random init (600) & 0.7741 (0.0017) \\
1000 & Essential hypertension & GRU, max pool, random init (300) & 0.7662 (0.0008) \\
1000 & Essential hypertension & GRU, max pool, PubMed init (500) & 0.7637 (0.0011) \\
1000 & Essential hypertension & Baseline - Bag of Words (15000) & 0.6902 (0.0019) \\
1000 & Essential hypertension & MCEMJ; min, mean, max pool (600) & 0.7086 (0.0014) \\
1000 & Essential hypertension & GloVe 300; min, mean, max pool (900) & 0.7045 (0.0016) \\
1000 & Essential hypertension & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7104 (0.0013) \\
1000 & Essential hypertension & GloVe 500; min, mean, max pool (1500) & 0.7057 (0.0019) \\
1000 & Essential hypertension & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7141 (0.0016) \\
1000 & Essential hypertension & LDA; max pool (300) & 0.6681 (0.0016) \\
1000 & Essential hypertension & LDA; max and mean pool (600) & 0.6703 (0.0016) \\
1000 & Essential hypertension & LDA; mean pool (300) & 0.6133 (0.0062) \\
1000 & Thyroid disorders & GRU, max pool, PubMed init (200) & 0.7148 (0.0017) \\
1000 & Thyroid disorders & GRU, max pool, random init (600) & 0.7667 (0.0023) \\
1000 & Thyroid disorders & GRU, max pool, random init (300) & 0.7532 (0.0019) \\
1000 & Thyroid disorders & GRU, max pool, PubMed init (500) & 0.6998 (0.0015) \\
1000 & Thyroid disorders & Baseline - Bag of Words (15000) & 0.6687 (0.0021) \\
1000 & Thyroid disorders & MCEMJ; min, mean, max pool (600) & 0.7268 (0.0016) \\
1000 & Thyroid disorders & GloVe 300; min, mean, max pool (900) & 0.6823 (0.0019) \\
1000 & Thyroid disorders & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7128 (0.0019) \\
1000 & Thyroid disorders & GloVe 500; min, mean, max pool (1500) & 0.6945 (0.0018) \\
1000 & Thyroid disorders & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7134 (0.0015) \\
1000 & Thyroid disorders & LDA; max pool (300) & 0.6219 (0.0019) \\
1000 & Thyroid disorders & LDA; max and mean pool (600) & 0.6293 (0.0023) \\
1000 & Thyroid disorders & LDA; mean pool (300) & 0.5721 (0.0036) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
2000 & Mortality & GRU, max pool, PubMed init (200) & 0.8624 (0.0004) \\
2000 & Mortality & GRU, max pool, random init (600) & 0.8792 (0.0004) \\
2000 & Mortality & GRU, max pool, random init (300) & 0.877 (0.0004) \\
2000 & Mortality & GRU, max pool, PubMed init (500) & 0.8612 (0.0005) \\
2000 & Mortality & Baseline - Bag of Words (15000) & 0.894 (0.001) \\
2000 & Mortality & MCEMJ; min, mean, max pool (600) & 0.8744 (0.0006) \\
2000 & Mortality & GloVe 300; min, mean, max pool (900) & 0.8839 (0.0006) \\
2000 & Mortality & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.8934 (0.0006) \\
2000 & Mortality & GloVe 500; min, mean, max pool (1500) & 0.8914 (0.0009) \\
2000 & Mortality & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.8661 (0.001) \\
2000 & Mortality & LDA; max pool (300) & 0.8486 (0.0007) \\
2000 & Mortality & LDA; max and mean pool (600) & 0.8483 (0.0004) \\
2000 & Mortality & LDA; mean pool (300) & 0.8089 (0.0009) \\
2000 & ER visit & GRU, max pool, PubMed init (200) & 0.7737 (0.0005) \\
2000 & ER visit & GRU, max pool, random init (600) & 0.7817 (0.0005) \\
2000 & ER visit & GRU, max pool, random init (300) & 0.7757 (0.0008) \\
2000 & ER visit & GRU, max pool, PubMed init (500) & 0.7723 (0.0005) \\
2000 & ER visit & Baseline - Bag of Words (15000) & 0.7759 (0.0007) \\
2000 & ER visit & MCEMJ; min, mean, max pool (600) & 0.7805 (0.0009) \\
2000 & ER visit & GloVe 300; min, mean, max pool (900) & 0.782 (0.0006) \\
2000 & ER visit & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7867 (0.0007) \\
2000 & ER visit & GloVe 500; min, mean, max pool (1500) & 0.7848 (0.0008) \\
2000 & ER visit & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.787 (0.0004) \\
2000 & ER visit & LDA; max pool (300) & 0.7368 (0.0014) \\
2000 & ER visit & LDA; max and mean pool (600) & 0.7497 (0.0011) \\
2000 & ER visit & LDA; mean pool (300) & 0.7334 (0.0011) \\
2000 & Inpatient Admission & GRU, max pool, PubMed init (200) & 0.7938 (0.0006) \\
2000 & Inpatient Admission & GRU, max pool, random init (600) & 0.8034 (0.0007) \\
2000 & Inpatient Admission & GRU, max pool, random init (300) & 0.8008 (0.0008) \\
2000 & Inpatient Admission & GRU, max pool, PubMed init (500) & 0.7882 (0.0009) \\
2000 & Inpatient Admission & Baseline - Bag of Words (15000) & 0.7944 (0.0009) \\
2000 & Inpatient Admission & MCEMJ; min, mean, max pool (600) & 0.7906 (0.0006) \\
2000 & Inpatient Admission & GloVe 300; min, mean, max pool (900) & 0.7942 (0.0007) \\
2000 & Inpatient Admission & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7996 (0.0007) \\
2000 & Inpatient Admission & GloVe 500; min, mean, max pool (1500) & 0.7974 (0.0008) \\
2000 & Inpatient Admission & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7944 (0.0008) \\
2000 & Inpatient Admission & LDA; max pool (300) & 0.7701 (0.0012) \\
2000 & Inpatient Admission & LDA; max and mean pool (600) & 0.7748 (0.0013) \\
2000 & Inpatient Admission & LDA; mean pool (300) & 0.7503 (0.0011) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
2000 & Cardiac dysrhythmias & GRU, max pool, PubMed init (200) & 0.7506 (0.001) \\
2000 & Cardiac dysrhythmias & GRU, max pool, random init (600) & 0.7629 (0.0009) \\
2000 & Cardiac dysrhythmias & GRU, max pool, random init (300) & 0.7638 (0.0008) \\
2000 & Cardiac dysrhythmias & GRU, max pool, PubMed init (500) & 0.7499 (0.0009) \\
2000 & Cardiac dysrhythmias & Baseline - Bag of Words (15000) & 0.7418 (0.001) \\
2000 & Cardiac dysrhythmias & MCEMJ; min, mean, max pool (600) & 0.7495 (0.0006) \\
2000 & Cardiac dysrhythmias & GloVe 300; min, mean, max pool (900) & 0.7431 (0.0007) \\
2000 & Cardiac dysrhythmias & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7544 (0.0007) \\
2000 & Cardiac dysrhythmias & GloVe 500; min, mean, max pool (1500) & 0.7452 (0.0007) \\
2000 & Cardiac dysrhythmias & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7505 (0.001) \\
2000 & Cardiac dysrhythmias & LDA; max pool (300) & 0.6993 (0.0009) \\
2000 & Cardiac dysrhythmias & LDA; max and mean pool (600) & 0.7025 (0.0011) \\
2000 & Cardiac dysrhythmias & LDA; mean pool (300) & 0.6734 (0.0013) \\
2000 & Diabetes mellitus w/o complic. & GRU, max pool, PubMed init (200) & 0.7741 (0.0007) \\
2000 & Diabetes mellitus w/o complic. & GRU, max pool, random init (600) & 0.7994 (0.0008) \\
2000 & Diabetes mellitus w/o complic. & GRU, max pool, random init (300) & 0.7829 (0.0006) \\
2000 & Diabetes mellitus w/o complic. & GRU, max pool, PubMed init (500) & 0.7672 (0.0007) \\
2000 & Diabetes mellitus w/o complic. & Baseline - Bag of Words (15000) & 0.7499 (0.002) \\
2000 & Diabetes mellitus w/o complic. & MCEMJ; min, mean, max pool (600) & 0.7592 (0.0011) \\
2000 & Diabetes mellitus w/o complic. & GloVe 300; min, mean, max pool (900) & 0.7408 (0.0011) \\
2000 & Diabetes mellitus w/o complic. & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7625 (0.0009) \\
2000 & Diabetes mellitus w/o complic. & GloVe 500; min, mean, max pool (1500) & 0.7452 (0.0011) \\
2000 & Diabetes mellitus w/o complic. & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7481 (0.0017) \\
2000 & Diabetes mellitus w/o complic. & LDA; max pool (300) & 0.6921 (0.0014) \\
2000 & Diabetes mellitus w/o complic. & LDA; max and mean pool (600) & 0.6984 (0.0013) \\
2000 & Diabetes mellitus w/o complic. & LDA; mean pool (300) & 0.6464 (0.0012) \\
2000 & Spondylosis (back pain) & GRU, max pool, PubMed init (200) & 0.7609 (0.0008) \\
2000 & Spondylosis (back pain) & GRU, max pool, random init (600) & 0.7732 (0.0005) \\
2000 & Spondylosis (back pain) & GRU, max pool, random init (300) & 0.7662 (0.0008) \\
2000 & Spondylosis (back pain) & GRU, max pool, PubMed init (500) & 0.7519 (0.0004) \\
2000 & Spondylosis (back pain) & Baseline - Bag of Words (15000) & 0.7286 (0.0009) \\
2000 & Spondylosis (back pain) & MCEMJ; min, mean, max pool (600) & 0.7342 (0.0011) \\
2000 & Spondylosis (back pain) & GloVe 300; min, mean, max pool (900) & 0.7393 (0.0009) \\
2000 & Spondylosis (back pain) & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7453 (0.0009) \\
2000 & Spondylosis (back pain) & GloVe 500; min, mean, max pool (1500) & 0.7409 (0.0011) \\
2000 & Spondylosis (back pain) & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7403 (0.0009) \\
2000 & Spondylosis (back pain) & LDA; max pool (300) & 0.6971 (0.0007) \\
2000 & Spondylosis (back pain) & LDA; max and mean pool (600) & 0.7027 (0.0009) \\
2000 & Spondylosis (back pain) & LDA; mean pool (300) & 0.6482 (0.0011) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
2000 & Disorders of lipid metabolism & GRU, max pool, PubMed init (200) & 0.7523 (0.001) \\
2000 & Disorders of lipid metabolism & GRU, max pool, random init (600) & 0.7624 (0.0009) \\
2000 & Disorders of lipid metabolism & GRU, max pool, random init (300) & 0.7596 (0.0009) \\
2000 & Disorders of lipid metabolism & GRU, max pool, PubMed init (500) & 0.7428 (0.001) \\
2000 & Disorders of lipid metabolism & Baseline - Bag of Words (15000) & 0.7106 (0.0015) \\
2000 & Disorders of lipid metabolism & MCEMJ; min, mean, max pool (600) & 0.7149 (0.0011) \\
2000 & Disorders of lipid metabolism & GloVe 300; min, mean, max pool (900) & 0.7086 (0.0013) \\
2000 & Disorders of lipid metabolism & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7221 (0.0011) \\
2000 & Disorders of lipid metabolism & GloVe 500; min, mean, max pool (1500) & 0.7107 (0.0012) \\
2000 & Disorders of lipid metabolism & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7163 (0.0011) \\
2000 & Disorders of lipid metabolism & LDA; max pool (300) & 0.6545 (0.0013) \\
2000 & Disorders of lipid metabolism & LDA; max and mean pool (600) & 0.6628 (0.0017) \\
2000 & Disorders of lipid metabolism & LDA; mean pool (300) & 0.6219 (0.0014) \\
2000 & Essential hypertension & GRU, max pool, PubMed init (200) & 0.7758 (0.0008) \\
2000 & Essential hypertension & GRU, max pool, random init (600) & 0.7878 (0.0009) \\
2000 & Essential hypertension & GRU, max pool, random init (300) & 0.7759 (0.0011) \\
2000 & Essential hypertension & GRU, max pool, PubMed init (500) & 0.7737 (0.0005) \\
2000 & Essential hypertension & Baseline - Bag of Words (15000) & 0.7176 (0.0013) \\
2000 & Essential hypertension & MCEMJ; min, mean, max pool (600) & 0.7272 (0.0011) \\
2000 & Essential hypertension & GloVe 300; min, mean, max pool (900) & 0.7204 (0.0011) \\
2000 & Essential hypertension & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7328 (0.0008) \\
2000 & Essential hypertension & GloVe 500; min, mean, max pool (1500) & 0.7213 (0.0008) \\
2000 & Essential hypertension & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7259 (0.0012) \\
2000 & Essential hypertension & LDA; max pool (300) & 0.678 (0.0012) \\
2000 & Essential hypertension & LDA; max and mean pool (600) & 0.6824 (0.0014) \\
2000 & Essential hypertension & LDA; mean pool (300) & 0.6355 (0.0014) \\
2000 & Thyroid disorders & GRU, max pool, PubMed init (200) & 0.7281 (0.001) \\
2000 & Thyroid disorders & GRU, max pool, random init (600) & 0.7819 (0.0012) \\
2000 & Thyroid disorders & GRU, max pool, random init (300) & 0.769 (0.001) \\
2000 & Thyroid disorders & GRU, max pool, PubMed init (500) & 0.713 (0.0011) \\
2000 & Thyroid disorders & Baseline - Bag of Words (15000) & 0.7008 (0.0022) \\
2000 & Thyroid disorders & MCEMJ; min, mean, max pool (600) & 0.7482 (0.0013) \\
2000 & Thyroid disorders & GloVe 300; min, mean, max pool (900) & 0.7043 (0.0008) \\
2000 & Thyroid disorders & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7401 (0.0012) \\
2000 & Thyroid disorders & GloVe 500; min, mean, max pool (1500) & 0.7135 (0.001) \\
2000 & Thyroid disorders & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7264 (0.0015) \\
2000 & Thyroid disorders & LDA; max pool (300) & 0.6343 (0.0015) \\
2000 & Thyroid disorders & LDA; max and mean pool (600) & 0.6451 (0.0014) \\
2000 & Thyroid disorders & LDA; mean pool (300) & 0.5896 (0.0049) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
4000 & Mortality & GRU, max pool, PubMed init (200) & 0.8661 (0.0002) \\
4000 & Mortality & GRU, max pool, random init (600) & 0.8831 (0.0003) \\
4000 & Mortality & GRU, max pool, random init (300) & 0.8801 (0.0003) \\
4000 & Mortality & GRU, max pool, PubMed init (500) & 0.866 (0.0003) \\
4000 & Mortality & Baseline - Bag of Words (15000) & 0.907 (0.0005) \\
4000 & Mortality & MCEMJ; min, mean, max pool (600) & 0.882 (0.0005) \\
4000 & Mortality & GloVe 300; min, mean, max pool (900) & 0.8921 (0.0006) \\
4000 & Mortality & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.9015 (0.0006) \\
4000 & Mortality & GloVe 500; min, mean, max pool (1500) & 0.9002 (0.0006) \\
4000 & Mortality & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.9078 (0.0006) \\
4000 & Mortality & LDA; max pool (300) & 0.8558 (0.0007) \\
4000 & Mortality & LDA; max and mean pool (600) & 0.8584 (0.0006) \\
4000 & Mortality & LDA; mean pool (300) & 0.8189 (0.0006) \\
4000 & ER visit & GRU, max pool, PubMed init (200) & 0.7763 (0.0005) \\
4000 & ER visit & GRU, max pool, random init (600) & 0.7858 (0.0005) \\
4000 & ER visit & GRU, max pool, random init (300) & 0.7791 (0.0005) \\
4000 & ER visit & GRU, max pool, PubMed init (500) & 0.7761 (0.0003) \\
4000 & ER visit & Baseline - Bag of Words (15000) & 0.7836 (0.0006) \\
4000 & ER visit & MCEMJ; min, mean, max pool (600) & 0.7871 (0.0005) \\
4000 & ER visit & GloVe 300; min, mean, max pool (900) & 0.7873 (0.0007) \\
4000 & ER visit & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7927 (0.0006) \\
4000 & ER visit & GloVe 500; min, mean, max pool (1500) & 0.7912 (0.0006) \\
4000 & ER visit & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7947 (0.0006) \\
4000 & ER visit & LDA; max pool (300) & 0.7443 (0.0006) \\
4000 & ER visit & LDA; max and mean pool (600) & 0.7594 (0.0005) \\
4000 & ER visit & LDA; mean pool (300) & 0.7414 (0.0008) \\
4000 & Inpatient Admission & GRU, max pool, PubMed init (200) & 0.7995 (0.0004) \\
4000 & Inpatient Admission & GRU, max pool, random init (600) & 0.8111 (0.0005) \\
4000 & Inpatient Admission & GRU, max pool, random init (300) & 0.8069 (0.0004) \\
4000 & Inpatient Admission & GRU, max pool, PubMed init (500) & 0.7939 (0.0003) \\
4000 & Inpatient Admission & Baseline - Bag of Words (15000) & 0.8062 (0.0006) \\
4000 & Inpatient Admission & MCEMJ; min, mean, max pool (600) & 0.7989 (0.0005) \\
4000 & Inpatient Admission & GloVe 300; min, mean, max pool (900) & 0.8027 (0.0005) \\
4000 & Inpatient Admission & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.8085 (0.0005) \\
4000 & Inpatient Admission & GloVe 500; min, mean, max pool (1500) & 0.8053 (0.0005) \\
4000 & Inpatient Admission & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.8099 (0.0005) \\
4000 & Inpatient Admission & LDA; max pool (300) & 0.7801 (0.0006) \\
4000 & Inpatient Admission & LDA; max and mean pool (600) & 0.7864 (0.0006) \\
4000 & Inpatient Admission & LDA; mean pool (300) & 0.7615 (0.0005) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
4000 & Cardiac dysrhythmias & GRU, max pool, PubMed init (200) & 0.7559 (0.0005) \\
4000 & Cardiac dysrhythmias & GRU, max pool, random init (600) & 0.7718 (0.0005) \\
4000 & Cardiac dysrhythmias & GRU, max pool, random init (300) & 0.7675 (0.0005) \\
4000 & Cardiac dysrhythmias & GRU, max pool, PubMed init (500) & 0.7536 (0.0005) \\
4000 & Cardiac dysrhythmias & Baseline - Bag of Words (15000) & 0.756 (0.0009) \\
4000 & Cardiac dysrhythmias & MCEMJ; min, mean, max pool (600) & 0.7577 (0.0007) \\
4000 & Cardiac dysrhythmias & GloVe 300; min, mean, max pool (900) & 0.7523 (0.0006) \\
4000 & Cardiac dysrhythmias & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7617 (0.0007) \\
4000 & Cardiac dysrhythmias & GloVe 500; min, mean, max pool (1500) & 0.7549 (0.0005) \\
4000 & Cardiac dysrhythmias & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7629 (0.0005) \\
4000 & Cardiac dysrhythmias & LDA; max pool (300) & 0.7086 (0.001) \\
4000 & Cardiac dysrhythmias & LDA; max and mean pool (600) & 0.7135 (0.0009) \\
4000 & Cardiac dysrhythmias & LDA; mean pool (300) & 0.6808 (0.0008) \\
4000 & Diabetes mellitus w/o complic. & GRU, max pool, PubMed init (200) & 0.7816 (0.0006) \\
4000 & Diabetes mellitus w/o complic. & GRU, max pool, random init (600) & 0.8076 (0.0007) \\
4000 & Diabetes mellitus w/o complic. & GRU, max pool, random init (300) & 0.7909 (0.0004) \\
4000 & Diabetes mellitus w/o complic. & GRU, max pool, PubMed init (500) & 0.7746 (0.0006) \\
4000 & Diabetes mellitus w/o complic. & Baseline - Bag of Words (15000) & 0.7741 (0.0011) \\
4000 & Diabetes mellitus w/o complic. & MCEMJ; min, mean, max pool (600) & 0.775 (0.0009) \\
4000 & Diabetes mellitus w/o complic. & GloVe 300; min, mean, max pool (900) & 0.7557 (0.0009) \\
4000 & Diabetes mellitus w/o complic. & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7796 (0.0008) \\
4000 & Diabetes mellitus w/o complic. & GloVe 500; min, mean, max pool (1500) & 0.7638 (0.0008) \\
4000 & Diabetes mellitus w/o complic. & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7814 (0.0008) \\
4000 & Diabetes mellitus w/o complic. & LDA; max pool (300) & 0.7037 (0.0009) \\
4000 & Diabetes mellitus w/o complic. & LDA; max and mean pool (600) & 0.7129 (0.001) \\
4000 & Diabetes mellitus w/o complic. & LDA; mean pool (300) & 0.6578 (0.0014) \\
4000 & Spondylosis (back pain) & GRU, max pool, PubMed init (200) & 0.7644 (0.0003) \\
4000 & Spondylosis (back pain) & GRU, max pool, random init (600) & 0.7776 (0.0003) \\
4000 & Spondylosis (back pain) & GRU, max pool, random init (300) & 0.7708 (0.0003) \\
4000 & Spondylosis (back pain) & GRU, max pool, PubMed init (500) & 0.7556 (0.0004) \\
4000 & Spondylosis (back pain) & Baseline - Bag of Words (15000) & 0.7429 (0.0008) \\
4000 & Spondylosis (back pain) & MCEMJ; min, mean, max pool (600) & 0.7442 (0.0007) \\
4000 & Spondylosis (back pain) & GloVe 300; min, mean, max pool (900) & 0.749 (0.0008) \\
4000 & Spondylosis (back pain) & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7544 (0.0005) \\
4000 & Spondylosis (back pain) & GloVe 500; min, mean, max pool (1500) & 0.753 (0.0007) \\
4000 & Spondylosis (back pain) & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7577 (0.0008) \\
4000 & Spondylosis (back pain) & LDA; max pool (300) & 0.7046 (0.0006) \\
4000 & Spondylosis (back pain) & LDA; max and mean pool (600) & 0.7127 (0.0006) \\
4000 & Spondylosis (back pain) & LDA; mean pool (300) & 0.6624 (0.0011) \\
\bottomrule
\end{tabular}\\

\scriptsize
\noindent \begin{tabular}{rlll}
\toprule
N & Task & Model & AUROC (SEM) \\
\midrule
4000 & Disorders of lipid metabolism & GRU, max pool, PubMed init (200) & 0.7591 (0.0006) \\
4000 & Disorders of lipid metabolism & GRU, max pool, random init (600) & 0.7698 (0.0004) \\
4000 & Disorders of lipid metabolism & GRU, max pool, random init (300) & 0.7659 (0.0007) \\
4000 & Disorders of lipid metabolism & GRU, max pool, PubMed init (500) & 0.7491 (0.0006) \\
4000 & Disorders of lipid metabolism & Baseline - Bag of Words (15000) & 0.7365 (0.001) \\
4000 & Disorders of lipid metabolism & MCEMJ; min, mean, max pool (600) & 0.7294 (0.0008) \\
4000 & Disorders of lipid metabolism & GloVe 300; min, mean, max pool (900) & 0.7227 (0.0006) \\
4000 & Disorders of lipid metabolism & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.739 (0.0007) \\
4000 & Disorders of lipid metabolism & GloVe 500; min, mean, max pool (1500) & 0.7262 (0.0007) \\
4000 & Disorders of lipid metabolism & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7381 (0.0008) \\
4000 & Disorders of lipid metabolism & LDA; max pool (300) & 0.6674 (0.0014) \\
4000 & Disorders of lipid metabolism & LDA; max and mean pool (600) & 0.6789 (0.0013) \\
4000 & Disorders of lipid metabolism & LDA; mean pool (300) & 0.6388 (0.001) \\
4000 & Essential hypertension & GRU, max pool, PubMed init (200) & 0.7825 (0.0005) \\
4000 & Essential hypertension & GRU, max pool, random init (600) & 0.7961 (0.0006) \\
4000 & Essential hypertension & GRU, max pool, random init (300) & 0.7838 (0.0004) \\
4000 & Essential hypertension & GRU, max pool, PubMed init (500) & 0.7815 (0.0006) \\
4000 & Essential hypertension & Baseline - Bag of Words (15000) & 0.7432 (0.0011) \\
4000 & Essential hypertension & MCEMJ; min, mean, max pool (600) & 0.7364 (0.0008) \\
4000 & Essential hypertension & GloVe 300; min, mean, max pool (900) & 0.7325 (0.0007) \\
4000 & Essential hypertension & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7466 (0.0007) \\
4000 & Essential hypertension & GloVe 500; min, mean, max pool (1500) & 0.7355 (0.0008) \\
4000 & Essential hypertension & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7462 (0.0008) \\
4000 & Essential hypertension & LDA; max pool (300) & 0.6913 (0.0007) \\
4000 & Essential hypertension & LDA; max and mean pool (600) & 0.6988 (0.0009) \\
4000 & Essential hypertension & LDA; mean pool (300) & 0.6479 (0.0012) \\
4000 & Thyroid disorders & GRU, max pool, PubMed init (200) & 0.7392 (0.0006) \\
4000 & Thyroid disorders & GRU, max pool, random init (600) & 0.7934 (0.0008) \\
4000 & Thyroid disorders & GRU, max pool, random init (300) & 0.7773 (0.0007) \\
4000 & Thyroid disorders & GRU, max pool, PubMed init (500) & 0.7234 (0.0006) \\
4000 & Thyroid disorders & Baseline - Bag of Words (15000) & 0.7301 (0.0021) \\
4000 & Thyroid disorders & MCEMJ; min, mean, max pool (600) & 0.7641 (0.001) \\
4000 & Thyroid disorders & GloVe 300; min, mean, max pool (900) & 0.7169 (0.0008) \\
4000 & Thyroid disorders & GloVe 300 + MCEMJ; min, mean, max pool (1500) & 0.7592 (0.0008) \\
4000 & Thyroid disorders & GloVe 500; min, mean, max pool (1500) & 0.7281 (0.0006) \\
4000 & Thyroid disorders & GloVe 500 + MCEMJ; min, mean, max pool (2100) & 0.7585 (0.0008) \\
4000 & Thyroid disorders & LDA; max pool (300) & 0.6455 (0.0012) \\
4000 & Thyroid disorders & LDA; max and mean pool (600) & 0.6585 (0.001) \\
4000 & Thyroid disorders & LDA; mean pool (300) & 0.6061 (0.0013) \\
\bottomrule
\end{tabular}\\


==> sections/instructions.tex <==
\section{Submission of papers to NIPS 2013}

NIPS requires electronic submissions.  The electronic submission site is  
\begin{center}
   \url{http://papers.nips.cc}
\end{center}

Please read carefully the
instructions below, and follow them faithfully.
\subsection{Style}

Papers to be submitted to NIPS 2013 must be prepared according to the
instructions presented here. Papers may be only up to eight pages long,
including figures. Since 2009 an additional ninth page \textit{containing only
cited references} is allowed. Papers that exceed nine pages will not be
reviewed, or in any other way considered for presentation at the conference.
%This is a strict upper bound. 

Please note that this year we have introduced automatic line number generation
into the style file (for \LaTeXe and Word versions). This is to help reviewers
refer to specific lines of the paper when they make their comments. Please do
NOT refer to these line numbers in your paper as they will be removed from the
style file for the final version of accepted papers.

The margins in 2013 are the same as since 2007, which allow for $\approx 15\%$
more words in the paper compared to earlier years. We are also again using 
double-blind reviewing. Both of these require the use of new style files.

Authors are required to use the NIPS \LaTeX{} style files obtainable at the
NIPS website as indicated below. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

%% \subsection{Double-blind reviewing}

%% This year we are doing double-blind reviewing: the reviewers will not know 
%% who the authors of the paper are. For submission, the NIPS style file will 
%% automatically anonymize the author list at the beginning of the paper.

%% Please write your paper in such a way to preserve anonymity. Refer to
%% previous work by the author(s) in the third person, rather than first
%% person. Do not provide Web links to supporting material at an identifiable
%% web site.

%%\subsection{Electronic submission}
%%
%% \textbf{THE SUBMISSION DEADLINE IS MAY 31st, 2013. SUBMISSIONS MUST BE LOGGED BY
%% 23:00, MAY 31st, 2013, UNIVERSAL TIME}

%% You must enter your submission in the electronic submission form available at
%% the NIPS website listed above. You will be asked to enter paper title, name of
%% all authors, keyword(s), and data about the contact
%% author (name, full address, telephone, fax, and email). You will need to
%% upload an electronic (postscript or pdf) version of your paper.

%% You can upload more than one version of your paper, until the
%% submission deadline. We strongly recommended uploading your paper in
%% advance of the deadline, so you can avoid last-minute server congestion.
%%
%% Note that your submission is only valid if you get an e-mail
%% confirmation from the server. If you do not get such an e-mail, please
%% try uploading again. 


\subsection{Retrieval of style files}

The style files for NIPS and other conference information are available on the World Wide Web at
\begin{center}
   \url{http://www.nips.cc/}
\end{center}
The file \verb+nips2013.pdf+ contains these 
instructions and illustrates the
various formatting requirements your NIPS paper must satisfy. \LaTeX{}
users can choose between two style files:
\verb+nips11submit_09.sty+ (to be used with \LaTeX{} version 2.09) and
\verb+nips11submit_e.sty+ (to be used with \LaTeX{}2e). The file
\verb+nips2013.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own. The file
\verb+nips2013.rtf+ is provided as a shell for MS Word users.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

%% \subsection{Keywords for paper submission}
%% Your NIPS paper can be submitted with any of the following keywords (more than one keyword is possible for each paper):

%% \begin{verbatim}
%% Bioinformatics
%% Biological Vision
%% Brain Imaging and Brain Computer Interfacing
%% Clustering
%% Cognitive Science
%% Control and Reinforcement Learning
%% Dimensionality Reduction and Manifolds
%% Feature Selection
%% Gaussian Processes
%% Graphical Models
%% Hardware Technologies
%% Kernels
%% Learning Theory
%% Machine Vision
%% Margins and Boosting
%% Neural Networks
%% Neuroscience
%% Other Algorithms and Architectures
%% Other Applications
%% Semi-supervised Learning
%% Speech and Signal Processing
%% Text and Language Applications

%% \end{verbatim}

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, initial caps/lower case, bold, centered between
2~horizontal rules. Top rule is 4~points thick and bottom rule is 1~point
thick. Allow 1/4~inch space above and below title to rules. All pages should
start at 1~inch (6~picas) from the top of the page.

%The version of the paper submitted for review should have ``Anonymous Author(s)'' as the author of the paper.

For the final version, authors' names are
set in boldface, and each name is centered above the corresponding
address. The lead author's name is to be listed first (left-most), and
the co-authors' names (if different address) are set to follow. If
there is only one co-author, list both author and co-author side by side.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

First level headings are lower case (except for first word and proper nouns),
flush left, bold and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are lower case (except for first word and proper nouns),
flush left, bold and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are lower case (except for first word and proper nouns),
flush left, bold and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be numbered consecutively. The corresponding
number is to appear enclosed in square brackets, such as [1] or [2]-[5]. The
corresponding references are to be listed in the same order at the end of the
paper, in the \textbf{References} section. (Note: the standard
\textsc{Bib\TeX} style \texttt{unsrt} produces this.) As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

As submission is double blind, refer to your own published work in the 
third person. That is, use ``In the previous work of Jones et al.\ [4]'',
not ``In our previous work [4]''. If you cite your other papers that
are not widely available (e.g.\ a journal paper under review), use
anonymous author names in the citation, e.g.\ an author of the
form ``A.\ Anonymous''. 


\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures. 
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Fonts were the main cause of problems in the past years. Your PDF file must
only contain Type 1 or Embedded TrueType fonts. Here are a few instructions
to achieve this.

\begin{itemize}

\item You can check which fonts a PDF files uses.  In Acrobat Reader,
select the menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
available out-of-the-box on most Linux machines.

\item The IEEE has recommendations for generating PDF files whose fonts
are also acceptable for NIPS. Please see
\url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}

\item LaTeX users:

\begin{itemize}

\item Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user). 
PDF figures must be substituted for EPS figures, however.

\item Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim} 
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

Check that the PDF files only contains Type 1 fonts. 
%For the final version, please send us both the Postscript file and
%the PDF file. 

\item xfig "patterned" shapes are implemented with 
bitmap fonts.  Use "solid" shapes instead. 
\item The \verb+\bbold+ package almost always uses bitmap
fonts.  You can try the equivalent AMS Fonts with command
\begin{verbatim}
\usepackage[psamsfonts]{amssymb}
\end{verbatim}
 or use the following workaround for reals, natural and complex: 
\begin{verbatim}
\newcommand{\RR}{I\!\!R} %real numbers
\newcommand{\Nat}{I\!\!N} %natural numbers 
\newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}

\item Sometimes the problematic fonts are used in figures
included in LaTeX files. The ghostscript program \verb+eps2eps+ is the simplest
way to clean such figures. For black and white figures, slightly better
results can be achieved with program \verb+potrace+.
\end{itemize}
\item MSWord and Windows users (via PDF file):
\begin{itemize}
\item Install the Microsoft Save as PDF Office 2007 Add-in from
\url{http://www.microsoft.com/downloads/details.aspx?displaylang=en\&familyid=4d951911-3e7e-4ae6-b059-a2e79ed87041}
\item Select ``Save or Publish to PDF'' from the Office or File menu
\end{itemize}
\item MSWord and Mac OS X users (via PDF file):
\begin{itemize}
\item From the print menu, click the PDF drop-down box, and select ``Save
as PDF...''
\end{itemize}
\item MSWord and Windows users (via PS file):
\begin{itemize}
\item To create a new printer
on your computer, install the AdobePS printer driver and the Adobe Distiller PPD file from
\url{http://www.adobe.com/support/downloads/detail.jsp?ftpID=204} {\it Note:} You must reboot your PC after installing the
AdobePS driver for it to take effect.
\item To produce the ps file, select ``Print'' from the MS app, choose
the installed AdobePS printer, click on ``Properties'', click on ``Advanced.''
\item Set ``TrueType Font'' to be ``Download as Softfont''
\item Open the ``PostScript Options'' folder
\item Select ``PostScript Output Option'' to be ``Optimize for Portability''
\item Select ``TrueType Font Download Option'' to be ``Outline''
\item Select ``Send PostScript Error Handler'' to be ``No''
\item Click ``OK'' three times, print your file.
\item Now, use Adobe Acrobat Distiller or ps2pdf to create a PDF file from
the PS file. In Acrobat, check the option ``Embed all fonts'' if
applicable.
\end{itemize}

\end{itemize}
If your file contains Type 3 fonts or non embedded TrueType fonts, we will
ask you to fix it. 

\subsection{Margins in LaTeX}
 
Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ... 
   \includegraphics[width=0.8\linewidth]{myfile.eps} 
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ... 
   \includegraphics[width=0.8\linewidth]{myfile.pdf} 
\end{verbatim}
for .pdf graphics. 
See section 4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps}) 
 
A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.


==> sections/intrinsic_eval.tex <==
\subsection*{Intrinsic evaluation of word embeddings}
\label{sec:embd-eval}
In order to shed light on the effectiveness of our learned representations, we asked whether the geometric properties that have been used to evaluate the quality of word embeddings are correlated with the utility of representations for our target tasks. 
Word embeddings are typically evaluated using analogy-like tasks that
test whether or not the geometry of the word embeddings recapitulates
known relationships between words.  We evaluated the word level
embeddings learned from clinical text, research article abstracts, and
through the recurrent net models using the Medical Relatedness
Property framework developed in \citep{choi2016learning}.  In this
framework, we test whether word embeddings express known \emph{may
  treat} and \emph{may prevent} relationships between drugs and
indications using vector arithmetic.  For instance, if $d_1, d_2, m_1,
\textnormal{ and } m_2 $ denote two drugs and indications
respectively, and the relation $r$ holds for $(d_1, m_1)$ and $(d_2,
m_2)$, we check whether or not the following holds for their
respective embeddings:

\begin{align*}
e_{d_1} - e_{m_1} + e_{m_2} \approx e_{d_2}
\end{align*}

More precisely, the quality metric is the ratio of concepts for which
at least one of the top-40 neighbors of $e_{d_1} - e_{m_1} + e_{m_2}$
satisfies the relation $r$ with $m_2$.  Results are shown in
\autoref{tab:intrinsic}.

\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|}
\hline
\textbf{Embedding method} & \textbf{May-Treat  (\%)} & \textbf{May-Prevent (\%)}    \\ \hline
GloVe            & 9.23           & 10.21          \\ \hline
MCEMJ                        & 8.25           & 6.81           \\ \hline
GRU        & 1.26           & 0.43           \\ \hline
\end{tabular}
\caption{Evaluation of the Medical Relatedness Property for two
  relations: May-Treat and May-Prevent.  }
\label{tab:intrinsic}
\end{table}

Interestingly, we found that GloVe embeddings performed better than
the MCEMJ embeddings, despite randomized word orders and a
significantly larger vocabulary.  This suggests that, with respect to both this intrinsic evaluation and as a building block for patient level representations, it not necessarily advantageous to have access to full text.  In addition, embeddings from
randomly initialized neural models perform poorly at this task despite
their effectiveness in the patient level prediction tasks, suggesting
that word level evaluations are not particularly predictive of utility
in such tasks.  


==> sections/intro.tex <==
Longitudinal clinical data are complex and high dimensional.  Researchers must make challenging decisions that can have a significant impact on predictive performance and clinical findings when preparing the data for analysis.  \textit{Finding a good representation for clinical data} is a critical step in designing studies and constitutes a grand challenge for machine learning researchers interested in health care.

% The question of representation is especially salient
In this paper, we study how to learn good patient representations from clinical notes.
Notes record crucial details about patient care and expert insights that cannot be found elsewhere in electronic health records (EHRs), but they also present a number of challenges to health care researchers, including high dimensionality, sparsity, and complex temporal structure.  Furthermore, datasets for supervised learning are frequently quite small relative to the complexity of the input space.  Although the volume of data in EHRs is increasing over time, reliable labels remain a scarce resource because manual review of patient records by highly trained clinicians remains the gold standard for such labels.  A good representation of clinical text should directly mitigate or admit simple strategies for overcoming these challenges.  Specifically, it should admit high performance models learned from limited training data.  Moreover, it should be \textit{useful across a wide range of clinical prediction tasks and research questions} and require minimal task-specific customization.

We take a \emph{transfer learning} approach to constructing \textit{data-driven representations of clinical text} that address these challenges and overcome the shortcomings of text representations that are commonly used in clinical informatics research.  Transfer learning is an approach that has been used to achieve state of the art results in computer vision and Natural Language Process (NLP) on tasks with limited training data.  For such problems, the scarcity of training data presents a challenge to using high capacity models such as deep neural nets.  Transfer learning with neural nets addresses this problem by first training a high capacity neural net on a \emph{source task} with a very large dataset with abundant labels.  The resulting model is then either used as a fixed feature extractor or parts of the model are fine tuned for a new \emph{target task} with much more limited training data.  In effect, the source task is used to learn how to transform the inputs into a useful form, i.e., a good representation of the inputs, and that transformation is applied to new data for the target task with the hope that the representation is also good for the target task.  

We apply this paradigm to learning effective representations of clinical notes.  We take two approaches to the source problem, both based on commonly used deep learning techniques.  The first approach, \emph{embed and aggregate}, uses GloVe \citep{pennington2014glove} to learn low-dimensional, dense embeddings of clinical terms.  We then derive patient-level representations from the term embeddings using simple operations, e.g., max pooling, across individual notes and sequences of notes.  In the second approach, we use recurrent neural nets (RNNs) \citep{elman1990finding} with an embedding layer to directly learn hidden representations of terms, notes, and patients simultaneously.  Both source tasks are trained on a large corpus of clinical notes from Stanford Hospital.  The resulting representations are evaluated by using them as inputs to models for predicting a variety of complex clinical outcomes and diagnoses, fit to small training sets ranging in size from 125 to 4,000 patients.  Our patient embeddings outperformed baseline representations based on bag of words (BOW) and topic models by large margins for small training set sizes for all outcomes.

The remainder of this paper is organized as follows: we discuss the challenges and desiderata of effective representations of clinical text in greater detail in \autoref{sec:background}.  We describe our data, methods, and experimental results in \autoref{sec:data}, \autoref{sec:methods}, and \autoref{sec:experiments}, respectively.  We conclude with a discussion of related work (\autoref{sec:related}) and the implications and limitations of our work with an eye toward future work (\autoref{sec:discussion}).

% Patient-level representations are evaluated through multiple classification tasks of different complexity. These were designed to mimic real-world settings and tackle problems of interest for health-care providers.
% In particular we consider the problem of \textit{transfer learning} and train our models on a small number of patients (500 or 2,000), since labeling is complex and expensive, and thus bioinformaticians usually have relatively small sample sizes when looking at particular cohorts.

% and detailed in \ref{sec:embd-eval}. This is an intrinsic evaluation similar to the analogy task and aims at assessing how well the embeddings capture semantic relations.
% Note-level representations are evaluated through the prediction of 15 phenotypes such as \textit{Asthma} and \textit{Obesity}, using a publicly available dataset, as detailed in \ref{sec:note-eval}.



% These embeddings mitigate the sparsity problem by capturing the common context, rather than identities, of clinical terms.
% , and complex sequence models, such as a 
% In this way, the learned term embeddings provide the same representational flexibility as BOW.


% we use a combination of natural language processing and deep learning techniques to develop models that can learn embeddings of clinical terms and notes. We propose multiple models, and compare them on a wide range of evaluation tasks. Because of the particular structure described above, our model learns embeddings on three scales: word-level embeddings are pooled to create note-level embeddings, which are aggregated to create patient-level embeddings, representing a patient's medical history through his medical notes. We compare (1) models where embeddings are first learned on the word level using count-based and neural models, and then aggregated across notes, and (2) models where all three embeddings are learned jointly in a recurrent neural network.



% We use these evaluations to compare various approaches at extracting these note embeddings, and also discuss some particular design choices involved in those models.

% Traditional clinical research confronts this challenge using domain expertise to identify variables that are believed \textit{a priori} to be relevant.
% This process is labor intensive and does not make full use of the wealth of data in \textit{electronic health records} (EHRs), limiting the possibility of serendipitous discovery~\citep{yu2015jamia,lependu2013pharmacovigilance}.
% In recent years, 

% These small data sets pose a significant obstacle to researchers seeking to solve clinical problems using machine learning and data mining, which perform best when labeled training data are plentiful.

% As such, they pose a number challenges to predictive modeling and data mining.
% Standard clinical notes have no formal structure so important observations can appear anywhere in the text, often without a clear or consistent indication.
% The same condition or symptoms can be described in a variety of ways: tachycardia may alternatively be described as a rapid heart rate or arrhythmia.
% Alternatively, a clinician may simply imply the presence of tachycardia by listing an obviously abnormal heart rate, trusting her expert reader recognize it.
% Clinical notes also rife with specialized vocabulary, shorthand and abbreviations, and stylistic conventions that vary across not only institutional boundaries but even individual clinicians.



% With the rise of electronic health records (EHR), applying machine learning methods to patient data has raised a lot of attention over the past years, for problems such as survival analysis, causal effect inference, mortality prediction, etc. However, whereas the EHR data warehouses are usually enormous, a common setback often met by bioinformatics researchers is that populations quickly become scarce when restricted to cohorts of interest, rendering almost impossible using the raw high-dimensional data. To that extent, several attempts have been made in learning general-purpose representations from patient records, to make downstream predictions easier and more accurate.

% These records usually contain a large set of numerical features such as patient demographics (e.g. age, gender, ethnicity), lab measurements (e.g. blood gases, fluid balances, vital signs), binary indicators for diseases and medical procedures, as well as free-text clinical notes. While numerical fields can be straightforward to use in most machine learning models, there is no common ground on how to process clinical notes from physicians and nurses. Researchers often use general-purpose off-the-shelf techniques, such as fitting topic models or learning direct word representations. These techniques, besides being somewhat impractical from a computational standpoint, are very generic and do not leverage the particular structure of these notes. They are, for each patients, a sequence of un-ordered collections of words\footnote{The words are always un-ordered in the notes as a consequence of the anonymization and annotation pipeline in the annotator used in our dataset, which is quite widely spread.}.

==> sections/methods.tex <==
We approach learning to represent patient clinical notes in the
framework of transfer learning, in which we learn to represent a
patient's clinical notes on a \emph{source task}, and use the
resulting representations for new \emph{target tasks}.  We took two approaches to the source task, described in detail below.  

\subsection*{Embed and Aggregate}
In this approach, we break up the source task into two phases.  First,
we learn word embeddings using methods such as GloVe or word2vec.
These embeddings are then aggregated into patient level embeddings
using simple functions \textemdash min, mean, and max \textemdash
applied element-wise to the embedding dimensions.  Note that this
aggregation is over two levels \textemdash word embeddings are first
combined into note representations, and then into patient level
representations.  Neither phase uses external labels, and are
unsupervised.  We explored word embeddings learned from both clinical
text and from biomedical research article abstracts as detailed below.

\subsubsection*{GloVe embeddings learned from clinical notes}
We used GloVe to learn word embeddings from clinical text using a range
of dimensionality and context sizes.  
In order to overcome the loss of the ordering of words in our input corpus, we 
adopted a technique used for learning embeddings of
medical codes \citep{choi2015doctor, choi2016learning}, which are
naturally unordered, and represent each note in the training corpus using 2 random orderings
of its words.  We ran GloVe for 25 iterations.  

\subsubsection*{Word embeddings from research article abstracts}
We also evaluated word embeddings learned from 350,000 biomedical
journal article abstracts in \citep{de2014medical}.  Terms in the
abstract text were mapped to UMLS CUIs, and the embeddings were
learned using the word2vec skip-gram model with a window size of 5 and
dimensionality of 200.  Embeddings for 52,000 CUIs are publicly
available,\footnote{\url{https://github.com/clinicalml/embeddings}}
and approximately 28,000 of those are in our vocabulary.  We refer to
these embeddings as MCEMJ (Medical Concept Embeddings from Medical
Journals).  

\subsubsection*{Aggregation of word embeddings}
We constructed fixed length representations of the patients using
simple functions -- min, mean, and max -- applied element-wise to the
word embeddings within each note.  We explored a range of embedding
sizes, along with concatenation of embeddings resulting from different
aggregation methods, and concatenation of embeddings learned from
different data sources.

\subsection*{Recurrent neural nets}
In this approach, we use recurrent neural nets whose inputs are a
sequence of bag of words vectors representing the clinical notes from a
given patient's input era.  This approach jointly learns word-, note-,
and patient-level embeddings (figure \ref{fig:rnn_architecture}).  Models are trained using input era data
only and are then used as fixed feature extractors for the target
tasks.

\subsubsection*{Neural Net Supervision}
Supervision for the recurrent neural net source task was provided by
Clinical Classification Software
(CCS)\footnote{https://www.hcup-us.ahrq.gov/toolssoftware/ccs/ccs.jsp}
codes derived from structured diagnosis codes from each patient's input era.  CCS maps
12,856 diagnosis codes into 254 broad disease categories such as
\emph{lung cancer} or \emph{cardiac dysrhythmias}, and have previously
been used as supervision labels for the training of recurrent neural
nets \citep{choi2015doctor} because it dramatically reduces the label
space.  We formulated learning as a multi-task sequence
classification problem in which the final hidden state of the net 
is used as a representation for a multi-task problem with
CCS labels aggregated over the patient's input era.  In preliminary
experiments, this approach consistently outperformed
providing supervision at each step using only that encounter's codes.  

\subsubsection*{Architecture}

\begin{figure}[h]
\centering \includegraphics[width=0.9\textwidth]{figures/rnn.png}
\caption{Model architecture for the recurrent neural net.  The input at each timestep is a many-hot vector of the terms mentioned at that timestep, corresponding to a clinical note.  The model jointly learns an embedding for each term and a patient level representation for the sequence of inputs.  Supervision for the model is provided by diagnosis codes contemporaneous with the input notes.}
\label{fig:rnn_architecture}
\end{figure}

As in other work using recurrent nets to model patient data, the input
to our recurrent nets were many-hot vectors representing the unordered
bag of words for each note \citep{choi2015doctor}.  Typically, the
first layer of the network multiplies an embedding matrix by this
vector, effectively summing the embeddings to arrive at a note level
representation that is input to recurrent cells.  However, we found
that applying an element-wise maximum to the embeddings at each
time-step significantly improved performance in the target tasks.

%More
%precisely, the input to the recurrent cells for a note $x$ is given
%by:
%
%$$ \phi_L(x) = \text{max}_1(x \odot L) $$
%
%where $x=[0,0,1, ... ,0,1,0]$ is the note bag-of-words encoding of
%shape $(V,1)$, $L$ is the word embedding matrix of shape $(V, D_x)$
%($V$ being the vocabulary size and $D_x$ the word embedding size), and
%$\text{max}_1$ performs a max over the first dimension.  

Finally, we explored using Long Short-Term Memory (LSTM) 
\citep{hochreiter1997long} and Gated Recurrent Units (GRU)
\citep{cho2014learning} as recurrent cells.  We found that,
consistent with \citep{choi2015doctor}, GRUs consistently outperformed
LSTMs.  Thus, our final experiments used GRUs with max aggregation of word embeddings.  

\subsubsection*{Learning details}
We used \texttt{tanh} activations, dropout with drop probability 0.2,
and a dense layer with binary cross-entropies for the multi-task
supervision. Networks were trained with RMSProp
\citep{tieleman2012lecture} for 100 epochs using a batch size of 32 and
maximum sequence length of 50, with longer sequences truncated to keep
the most recent notes.  The models were implemented in Keras 1.2.0
\citep{chollet2015keras} with a Tensorflow 0.12.1 backend \citep{tensorflow}
on an NVIDIA GeForce GTX TITAN X GPU.  

We explored initializing the embedding layer of our recurrent nets
using word embeddings learned from the clinical notes or from from
research article abstracts.  We found that random initialization
consistently outperformed initialization with pre-trained embeddings. 

\subsection*{Baselines - Bag of words and topic models}
We compared the learned representations against BOW and topic model representations of words and notes respectively.  For the BOW experiments, we limited the vocabulary to the 15,000 most frequent
words in each training subsample.  Word counts were then summed over each patient's input notes.  The final representation consisted of TF-IDF transformed counts of words for each patient. Latent Dirichlet Allocation was used to fit a topic model on training notes using Gensim \citep{gensim}. 300 topics were fit over two passes through the training notes.  The model was then used to estimate topic distributions for validation and test set notes.  The topic distributions for each note were aggregated into patient-level representations using mean and max pooling.





==> sections/plots.tex <==
\newpage
% Figure with learning curves
\begin{figure}[H]
\subfloat[]{\includegraphics[scale=0.535]{figures/Cardiac_dysrhythmias.pdf}}
\label{fig:cardiac} \\
\subfloat[]{\includegraphics[scale=0.535]{figures/Mortality.pdf}}
\label{fig:mortality}
\caption{Target task performance as a function of training set size. (a) Cardiac dysrhythmia diagnosis. (b) Mortality. The dimensionality of each representation is in parentheses.}
\label{fig:results}
\end{figure}
\begin{figure}[H]
\subfloat[]{\includegraphics[scale=0.535]{figures/ER_visit.pdf}}
\label{fig:er} \\
\subfloat[]{\includegraphics[scale=0.535]{figures/Inpatient_Admission.pdf}}
\label{fig:admission}
\caption{Target task performance as a function of training set size. (a) Future ER visit. (b) Future admission.  The dimensionality of each representation is in parentheses.}
\label{fig:results2}
\end{figure}



==> unused/conclusion.tex <==
\section{Conclusion}

Limitations:
\begin{itemize}
\item we didn't have raw notes with actual sequential structure -- what are implications for each model? RNN could conceivably make use of that info, don't think it would affect embeddings much
\item how would these be impacted if we removed standard clinical preprocessing pipeline? Would probably degrade a little but how much? Also, if preprocessing is available, we should use it!
\item evaluations were all concerned with prediction -- how would these work for traditional clinical studies?
\item are our randomly sampled small data sets representative of clinical study cohorts (meeting narrowly defined criteria)?
\item how would these perform for clinician-assigned labels vs. common outcomes or "derived" labels
\item transfer to data from other hospitals?
\end{itemize}

Nitpicks (maybe don't discuss):
\begin{itemize}
\item larger data sets: use 10-fold cross validation to do lambda.1se instead of lambda.min, may disadvantage bag of words
\end{itemize}

Future work:
\begin{itemize}
\item learning common embedding space for other data types + notes
\item train RNN as autoencoder
\item interpretability?
\end{itemize}

We showed in this work that is possible to learn embeddings from patients' clinical notes, which can easily be transfered to considerably smaller populations for specific prediction and classification problems, using a particularly relevant and thorough set of evaluation tasks. We showed that such learned representations not only render those smaller problems computationally more tractable, they also have the ability to improve the accuracy of such predictions, by capturing more of the semantic information contained in the notes than baseline models.

Furthermore, we proved that recurrent neural network can learn representations that yield particularly good improvements on these evaluation tasks, by leveraging the sequential arrangements of the notes in a patient's history, provided the correct design choices are made. However, it is interesting to note that while our \textit{"embed and aggregate"} methods perform less well than our sequence models, they are way quicker to train, demand less tweaking, and can be transfered across institutions and sub-problems in a more flexible manner. It is also interesting to note that models that perform the best on our extrinsic tasks (which are realistically the most important) are not necessarily the ones yielding the best word embeddings according to our word-level evaluation.

There are future developments that could be made to this model. First, it would be interesting to develop a new expression of the \texttt{GloVe} or \texttt{word2vec} objective function that takes into account the specific structure of these notes (sample negated words during negative sampling, sample windows from the set of words at each iteration, etc.). Secondly, it would be worth exploring other options for the RNN supervision. Ideally, the labels would be less sparse and would only use the notes' content; so perfect labels would be some very high-level aggregation of the concepts present in the note.

==> unused/data_old.tex <==
\subsection{Presentation}\label{sec:pres}
We use patient data collected at Stanford Hospital in the Stanford Translation Research Integrated Database Environment (STRIDE) from 2009 through 2014.  This dataset comprises 
Throughout this work, we use the STRIDE dataset, which is an anonymized medical data extract used by the \textit{Stanford Shah Lab} (BMIR\footnote{Stanford Center for Biomedical Informatics}.). This dataset is extracted from the much larger \textit{Stanford Translational Research Integrated Database Environment} (\cite{lowe2009stride}), a clinical data warehouse.

This extract contains about 27 million notes, corresponding to 1,2 million patients, most of them being between 1998 and 2014. There are about 49 million visits, each them having multiple procedures and diagnoses.

\begin{figure}[h]
\centering
\includegraphics[width=0.25\textwidth]{notes.png}
\caption{Notes are collections of terms, ordered in a patient's history}
\end{figure}

The clinical notes in this particular extract are processed and annotated using the Open Biomedical Annotator (\cite{lependu2013pharmacovigilance}), which is a pretty standard practice. This process anonymizes the notes (rendering the words un-ordered), and converts each term to concept IDs (CUI), which we will sill refer to as words in the remaining of the paper. The annotated notes have the following structure:

\begin{itemize}
 \item each patient has a number of clinical notes, written sequentially and timestamped
 \item each note is a (un-ordered) collection of terms
 \item terms have been processed, such that it is annotated whether they are negated and/or refer to the patient's family history
 \item terms can be mapped (in a many-to-one relation) to medical concepts
% \item medical concepts are also annotated with respect to their semantic hierarchy, but we will likely not use this level of detail in our model, as this particular feature is not present in all medical text datasets.
\end{itemize}

Each notes can also be associated with a \textit{visit}, during which various diagnoses are made (through ICD9 codes). Those diagnoses can be mapped to more general diseases categories through the \textit{Clinical Classification Software} (CCS)\footnote{https://www.hcup-us.ahrq.gov/toolssoftware/ccs/ccs.jsp}. Thus, for each note, we can obtain a collection of CCS codes diagnosed at the same time as the note.


\subsection{Setup and pre-processing}

\subsubsection*{Vocabulary}
While it is common practice to discard all negated words (such as in \cite{miotto2016deep}), we decided to include them as extra words in the vocabulary, as we believe negations have a particular meaning in clinical notes. This means that each word in our vocabulary also has its negated counterpart.

This gave us about 265k words, with an extremely long tail, so we restricted our vocabulary to keep relevant words only. We removed words appearing in fewer than 50 notes, and those appearing in more than 10 million notes. This led us to a vocabulary size of 107,388.

\subsubsection*{Patient eras}
As most of our extrinsic evaluations consist of prediction on patients, we split each patient's records in two eras: the input era, and the target era. Records in the input era will be used to train our embeddings as well as inputs in evaluation tasks, whereas records in the target era will be used as prediction targets in evaluation tasks. 

For each patient, we isolated a 6-months span of interest for the target era, and we used the previous year as input era. For instance, a year of medical notes and their embeddings could be used to predict the development of various diseases for a patient in the 6 months following this year of data.

\subsubsection*{Data split}
Our dataset consists of 69,416 patients for training, 11,289 for validation and 34,524 for testing. These patients were filtered from the STRIDE database to satisfy practical constraints such as having at least a couple visits during the input / target eras and having at least one clinical note containing a word form our restricted vocabulary.


==> unused/data_old2.tex <==
\subsection*{Data}
We use patient data collected at Stanford Hospital from 2009 through 2014 in the Stanford Translational Research Integrated Database Environment (STRIDE).  Each patient’s data comprises a timestamped series of encounters with care providers at Stanford Hospital.  Encounters may generate both structured and unstructured data.  The structured data typically consists of discrete codes from controlled vocabularies for diagnoses, medications, and procedures, along with quantitative measurements such as vitals and laboratory measurements.  The unstructured data consists of the free text of clinical notes written by care providers documenting each encounter and other aspects of patient care.  In all, the initial dataset comprises over 49 million encounters and 27 million notes for 2 million patients.  However, the effective size of the dataset is much smaller after it has been filtered for usable data as describe below.

==> unused/experiments_old.tex <==
\subsection{Word-level evaluation}\label{sec:embd-eval}

We evaluate our word embeddings through the \textit{Medical Relatedness Property} developed in \cite{choi2016learning} \footnote{We used their code to compute this metrics, which is available at \url{https://github.com/clinicalml/embeddings}}.

\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|}
\hline
\textbf{Embedding method}             & \textbf{May-Treat  (\%)}    & \textbf{May-Prevent (\%)}    \\ \hline
GloVe300-W10-R1           & 7.83           & 8.51           \\ \hline
GloVe-100-W7-R2            & 6.01           & 08.09          \\ \hline
GloVe-300-W4-R2            & 8.81           & \textbf{10.64} \\ \hline
GloVe-300-W7-R2            & 8.25           & 10.21          \\ \hline
GloVe-500-W7-R2            & 9.23           & 10.21          \\ \hline
GloVe-300-W10-R2           & \textbf{10.49} & 9.79           \\ \hline
GloVe-300-W4-R3            & 6.57           & 7.23           \\ \hline
MCEMJ                        & 8.25           & 6.81           \\ \hline
Cross-channel                & 5.45           & 2.55           \\ \hline
MaxGRU200-MCEMJ & 7.27           & 5.53           \\ \hline
MaxGRU300        & 1.26           & 0.43           \\ \hline
\end{tabular}
\caption{Evaluation of the Medical Relatedness Property for two relations: May-Treat and May-Prevent. "GloVe-300-W10-R2" corresponds to GloVe embeddings trained on our clinical notes, with length 300, window size 10, and clinical notes repeated twice in the corpus. All GloVe models were run for 25 iterations. "MaxGRU200-MCEMJ" is a RNN with GRU cells, 200 cells, initialized with MCEMJ. This evaluation was computed with the code provided by \cite{choi2016learning}}
\label{my-label}
\end{table}

Interestingly, we notice that many of our GloVe embeddings perform better than the MCEMJ ones (learned from abstracts of medical journals), despite randomized word orders and a vocabulary twice as big.
In addition, embeddings from randomly initialized neural models perform worse, especially the RNN.

\subsection{Note-level evaluation}
\label{sec:note-eval}

To evaluate our note representations, we used the \texttt{i2b2} (Informatics for Integrating Biology to the Bedside) 2008 Obesity Challenge \cite{uzuner2009recognizing}. 
The publicly available dataset contains approximately 1,230 clinical notes and 15 phenotype targets such as \textit{Asthma} and \textit{Obesity}.  The dataset is divided in two: the \textit{textual task} for which labels are attributed from explicit mention in the notes; for the \textit{intuitive task} however, classification was done by using doctors' intuition and judgment.

% The publicly available dataset contains approximately 1,230 clinical notes (730 for training and 500 for testing) and 15 targets. The targets are phenotypes such as \textit{Asthma, Obesity}, etc \dots There are 4 possible classes for each target: Present, Absent, Questionable and Unmentioned. The dataset is divided in two sub-tasks which contain the same inputs/outputs but differ on the method used to label the data. The first one is the \textit{textual task} for which labels are attributed from explicit mention in the notes; for the \textit{intuitive task} however, classification was done by using doctors' intuition and judgment based on the clinical notes. The latter is thus supposed to be more complex and require a higher level semantic understanding of the input.

To align with this competition, we consider the micro-averaged F1\footnote{Which corresponds to summing counts (true positives, \dots) across classes, see \cite{uzuner2009recognizing} for details.} as our main metric. For simplicity, we will only report the average performance across the 15 targets. More details about this dataset and our approach is provided in Appendix \ref{sec:app-i2b2}. We used a raw bag-of-words encoding of the notes as baseline.

% The notes were processed with the Shah Lab annotator so that it had the exact same format as the notes in the STRIDE database. From the original training set, we randomly subsampled a validation set containing 20\% of the data. We extensively used it and some results are presented in appendix. In particular, it enabled us to select the best classification model: a Random Forest with 10 trees for the baseline representation (bag-of-words) and a $k$-Nearest Neighbors for all other inputs ($k$ was chosen by cross-validation on the remaining training data).

\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|}
\hline
\textbf{Embedding method}               & \textbf{Textual}        & \textbf{Intuitive}      \\ \hline
Baseline                       & \textbf{0,822} & \textbf{0,802} \\ \hline
GloVe-300-W7-R2         & 0,784          & 0,773          \\ \hline
GloVe-500-W7-R2        & 0,779          & 0,774          \\ \hline
MCEMJ                         & 0,776          & 0,765          \\ \hline
MaxGRU300     & \textbf{0,793} & \textbf{0,778} \\ \hline
MaxGru200-MCEMJ & 0,781          & 0,769          \\ \hline
\end{tabular}
\caption{Micro-averaged F1 scores averaged over the 15 targets of the i2b2 Obesity Challenge test set. All embeddings where aggregated among the notes by component-wise maximum.}
\label{table:i2b2-test}
\end{table}

Overall, we did not notice much disparity in the accuracies yielded by the different representations, although the baseline performed a bit better than all our dense features. We also observed that in general, aggregating the word representation in a note with the \texttt{max} operator yielded the best results (compared to \texttt{mean, min, sum}). Finally, we notice that the baseline had a larger drop in performance between the \textit{textual} task and the \textit{intuitive} one, compared to the models based on the word embeddings. This could mean that word embeddings become more robust when the target gets more complex. 


\subsection{Patient-level evaluation}

% The final evaluation, on the patient level, is more extrinsic as that they reproduce the actual settings in which such embeddings would be used. 

The final evaluation - at the patient level - consists of various real-world applications in which such embeddings could be used, and thus it is our extrinsic evaluation.
We look at the performance of various prediction tasks, using only the learned embeddings as input. Moreover, to replicate the common drawback of prediction tasks in healthcare in actual settings, where sample sizes for actual problems of interest are often relatively small, we only use small training sets (respectively 500 and 2,000 patients) to evaluate those prediction tasks (the results are then averaged over 20 trials).

The tasks we use are particularly relevant to bioinformatics scientists and healthcare providers. We use the embeddings to predict various events in the patient's "target era": mortality. future admission, future emergency visits (ER), future development of the 6 densest diseases in our training set (thyroid disorder, cardiac dysrhythmias, diabetes, spondylosis, disorder of lipid metabolism, and essential hypertension). 

All of our evaluation models were trained using Ridge logistic regression, cross-validated over 5 folds (using \texttt{glmnet}), on a per-training group basis. The results were further averaged over 20 sampled training groups.
All GloVe methods reported here use a window size of 7 and 2 resampling of the notes. In addition all aggregations of word embeddings (GloVe and MCEMJ) are concatenations of aggregations by maximum, minimum and average since this always improved the performance. 

The baseline is a Ridge logistic regression fit on a raw bag-of-words encoding of the patient history of notes, where the vocabulary is restricted to the most frequent words appearing in the small training set\footnote{This is the only way to have this model converge in a majority of cases.}. We only kept the results when the baselines converged, but this does not happen all the time, and would even more rarely with longer eras and more patients.

\subsubsection*{Results with 500 patients}
For each model, we report the resulting average and standard error of Area Under Receiver-Operator Curve (AUROC):

\begin{table}[H]
\centering
\captionsetup{justification=centering}
\setlength{\tabcolsep}{10pt}
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Method}             & \multicolumn{1}{l|}{\textbf{Death}} & \multicolumn{1}{l|}{\textbf{Admission}} & \multicolumn{1}{l|}{\textbf{ER Visit}} \\ \hline
Baseline  &    
0.801 (0.019)&	0.711 (0.019)&	0.698 (0.005)                                        \\ \hline
GloVe-300 + MCEMJ  & 0.811 (0.005)                       & 0.758 (0.002)                           & 0.756 (0.002)                          \\ \hline
GloVe-500  + MCEMJ & 0.809 (0.006)                       & 0.757 (0.003)                           & 0.755 (0.003)                          \\ \hline
MCEMJ              & 0.795 (0.004)                       & 0.74 (0.003)                            & 0.729 (0.004)                          \\ \hline
GloVe-300          & 0.797 (0.005)                       & 0.752 (0.003)                           & 0.752 (0.002)                          \\ \hline
GloVe-500          & 0.805 (0.005)                       & 0.752 (0.004)                           & 0.752 (0.003)                          \\ \hline
MaxGRU300          & \textbf{0.842 (0.003)}              & 0.723 (0.022)                           & 0.745 (0.005)                          \\ \hline
MaxGRU600          & 0.829 (0.017)                       & \textbf{0.765 (0.004)}                  & \textbf{0.759 (0.002)}                 \\ \hline
MaxGRU500-MCEMJ    & 0.812 (0.017)                       & 0.746 (0.006)                           & 0.747 (0.004)                          \\ \hline
MaxGRU200-MCEMJ    & 0.817 (0.017)                       & 0.75 (0.006)                            & 0.754 (0.002)                          \\ \hline
\end{tabular}
\caption{Evaluation on mortality and utilization prediction tasks. Reported metrics are mean and standard error of AUROC and across 20 small evaluations.}
\end{table}

\begin{table}[H]
\centering
\captionsetup{justification=centering}
% \setlength{\tabcolsep}{10pt}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\textbf{Methods}  & \textbf{Thyroid} & \textbf{Dysrhythmias} & \textbf{Diabetes}      & \textbf{Spondylosis}   & \textbf{LMD\footnote{Lipid metabolism disorder.}} & \textbf{Hypertension} \\ \hline
Baseline                  & 
0.610 (0.009) &	0.687 (0.01)	& 0.68 (0.005)	& 0.667 (0.017)	& 0.635 (0.011) & 	0.664 (0.009)
\\ \hline
GloVe-300 + MCEMJ & 0.632 (0.009)              & 0.69 (0.004)                  & 0.689 (0.004)          & 0.696 (0.004)          & 0.648 (0.009)                          & 0.679 (0.005)                   \\ \hline
GloVe-500 + MCEMJ & 0.648 (0.006)              & 0.689 (0.005)                 & 0.691 (0.003)          & 0.701 (0.004)          & 0.649 (0.009)                          & 0.667 (0.01)                    \\ \hline
MCEMJ             & 0.642 (0.01)               & 0.688 (0.004)                 & 0.69 (0.004)           & 0.688 (0.003)          & 0.651 (0.005)                          & 0.666 (0.01)                    \\ \hline
Glove-300         & 0.618 (0.008)              & 0.683 (0.005)                 & 0.683 (0.004)          & 0.689 (0.003)          & 0.649 (0.005)                          & 0.672 (0.005)                   \\ \hline
Glove-500         & 0.618 (0.01)               & 0.686 (0.004)                 & 0.683 (0.004)          & 0.693 (0.003)          & 0.642 (0.008)                          & 0.67 (0.004)                    \\ \hline
MaxGRU300         & 0.701 (0.011)              & \textbf{0.709 (0.017)}        & 0.737 (0.013)          & 0.732 (0.012)          & 0.7 (0.015)                            & \textbf{0.745 (0.003)}          \\ \hline
MaxGRU600         & \textbf{0.721 (0.004)}     & 0.673 (0.023)                 & \textbf{0.744 (0.013)} & \textbf{0.738 (0.013)} & 0.702 (0.016)                          & 0.735 (0.013)                   \\ \hline
MaxGRU500-MCEMJ   & 0.623 (0.013)              & 0.673 (0.02)                  & 0.718 (0.012)          & 0.725 (0.004)          & \textbf{0.706 (0.004)}                 & 0.739 (0.005)                   \\ \hline
MaxGRU200-MCEMJ   & 0.662 (0.01)               & 0.697 (0.016)                 & 0.705 (0.02)           & 0.728 (0.012)          & 0.703 (0.011)                          & 0.741 (0.003)                   \\ \hline
\end{tabular}
\caption{Evaluation on prediction of future diseases. Reported metrics are mean and standard error of AUROC and across 20 small evaluations. }
\end{table}

We can observe most models beat the baseline quite easily (which often did not converge when fitting these evaluation models), except on mortality prediction where it appears to perform particularly well. The sequence models achieve the best results, however it is unclear whether it is due to the training supervision or to the fact it captures the sequential semantic information in the notes. 

\subsubsection*{Results with 2,000 patients}
The results with 2,000 patients are reported in the appendix \ref{app:2000}. The baseline is not included since it could never converge (2,000 patients per training groups means more word features, at a level where \texttt{glmnet} could not converge).


==> unused/intro_old.tex <==
Longitudinal clinical data are complex and high dimensional.
Simply understanding the data can be difficult, and when preparing the data for analysis, researchers are required to make challenging decisions that can have a significant impact on predictive performance and clinical findings.
Confronting these questions, namely \textit{finding the right representation for clinical data}, is a critical step in designing studies and constitutes a grand challenge for machine learning researchers interested in health care.

The question of representation is especially salient in the context of free text clinical notes, which record critical details of patient care and expert insights that cannot be found elsewhere in electronic health records (EHRs).
Clinical text presents a number of challenges: for one, \textit{clinical text are intrinsically high dimensional} due to their diversity of topics, specialized vocabulary, and combinatorial nature.
Even simple representations like bag of words (BOW), i.e., counts over a predefined vocabulary, can yield input (feature) vectors with millions of dimensions.
Patient cohorts, on the other hand, commonly number in the tens to hundreds, even at hospitals with millions of digital records.\footnote{This is due in part to the fact that many clinical research questions define strict case and control definitions, limiting the number of patients available for inclusion in any one study.
However, there is also a dearth of labeled data in EHRs: many outcomes of interest, such as mortality, occur outside the hospital and are not observed.
Many diseases go undiagnosed for long periods of time, and many more diagnoses are not recorded in a consistent manner during the delivery of care.}
This invokes the ``curse of dimensionality,'' making statistical models difficult to train without aggressive dimensionality reduction or regularization.
% BOW is intuitive and has enjoyed widespread success within health care~\citep{} and without~\citep{}.
% However, BOW fails to fully address many of the challenges presented by clinical text, leading health informatics researchers to seek alternatives~\citep{halpern2012comparison,jung2015functional}.

In a related problem, \textit{clinical text data are also inherently sparse}: phrases describing important clinical concepts may occur in only a handful of records.
This makes it difficult to discover a reliable statistical relationship between an outcome and such phrases, as well as the concepts they denote.
This problem is exacerbated by \textit{noise and ambiguity in clinical text}: ``tachycardia'' may alternatively be described as a ``rapid heart rate'' or ``arrhythmia.''\footnote{Alternatively, a clinician may simply imply the presence of tachycardia by listing an obviously abnormal heart rate, trusting an expert reader will recognize it.}
One can easily imagine cases where, due to such ambiguity,
the common dimensionality reduction heuristic of discarding rare terms actually removes all mentions of an important concept.

\textit{Clinical notes also exhibit a hierarchical sequential structure}: a longitudinal patient record includes a time series of notes, each itself consisting of a sequence of words.
% Both types of sequences can have arbitrary length, and
This poses trade-off between simplicity and fidelity when choosing a representation:
directly modeling this ``sequence of sequences'' structure requires a complex model architecture and most likely a large amount of training data.
In contrast, representing a patient history as a BOW is simple and flexible but discards information about time and order.
There is a spectrum of choices between these extremes, but they often involve only slightly less complexity \citep{choi2015doctor} or ad hoc decisions about, e.g., windowing time \citep{schuler2016discovering}.

In this paper, we take a deep learning approach to constructing \textit{data-driven representations of clinical text} that address these challenges and overcome the weaknesses of the BOW baseline used widely in clinical informatics.
In particular, we use GloVe \citep{pennington2014glove} and long short-term memory recurrent neural networks (LSTM RNN) \citep{hochreiter1997long} to learn real-valued, dense embeddings of clinical terms, notes


The learned embeddings are much lower dimensional (500 in our best performing model) than BOW vectors and mitigate the sparsity problem by capturing the common context, rather than identities, of clinical terms.
We demonstrate how similarly low dimensional note and patient representations can be derived from the term embeddings using both simple operations, e.g., max pooling, and more complex sequential models, such as .
In this way, the learned term embeddings provide the same representational flexibility as BOW.

Finally, we show that the learned embeddings provide a fourth


we use a combination of natural language processing and deep learning techniques to develop models that can learn embeddings of clinical terms and notes. We propose multiple models, and compare them on a wide range of evaluation tasks. Because of the particular structure described above, our model learns embeddings on three scales: word-level embeddings are pooled to create note-level embeddings, which are aggregated to create patient-level embeddings, representing a patient's medical history through his medical notes. We compare (1) models where embeddings are first learned on the word level using count-based and neural models, and then aggregated across notes, and (2) models where all three embeddings are learned jointly in a recurrent neural network.

As we believe work on representation learning and embedding extraction is only as valuable as its evaluations, we also focused our efforts on designing relevant and thorough quantitative evaluations of our embeddings. Because of the three-scale structure of these embeddings, it is natural to evaluate them on three levels. \\
Word embeddings are evaluated through the \textit{Medical Relatedness Property} developed in~\cite{choi2016learning} and detailed in \ref{sec:embd-eval}. This is an intrinsic evaluation similar to the analogy task and aims at assessing how well the embeddings capture semantic relations. Note-level representations are evaluated through the prediction of 15 phenotypes such as \textit{Asthma} and \textit{Obesity}, using a publicly available dataset, as detailed in \ref{sec:note-eval}. Patient-level representations are evaluated through multiple classification tasks of different complexity. These were designed to mimic real-world settings and tackle problems of interest for health-care providers. In particular we consider the problem of \textit{transfer learning} and train our models on a small number of patients (500 or 2,000), since labeling is complex and expensive, and thus bioinformaticians usually have relatively small sample sizes when looking at particular cohorts.

We use these evaluations to compare various approaches at extracting these note embeddings, and also discuss some particular design choices involved in those models.

% Traditional clinical research confronts this challenge using domain expertise to identify variables that are believed \textit{a priori} to be relevant.
% This process is labor intensive and does not make full use of the wealth of data in \textit{electronic health records} (EHRs), limiting the possibility of serendipitous discovery~\citep{yu2015jamia,lependu2013pharmacovigilance}.
% In recent years, 

% These small data sets pose a significant obstacle to researchers seeking to solve clinical problems using machine learning and data mining, which perform best when labeled training data are plentiful.

% As such, they pose a number challenges to predictive modeling and data mining.
% Standard clinical notes have no formal structure so important observations can appear anywhere in the text, often without a clear or consistent indication.
% The same condition or symptoms can be described in a variety of ways: tachycardia may alternatively be described as a rapid heart rate or arrhythmia.
% Alternatively, a clinician may simply imply the presence of tachycardia by listing an obviously abnormal heart rate, trusting her expert reader recognize it.
% Clinical notes also rife with specialized vocabulary, shorthand and abbreviations, and stylistic conventions that vary across not only institutional boundaries but even individual clinicians.



% With the rise of electronic health records (EHR), applying machine learning methods to patient data has raised a lot of attention over the past years, for problems such as survival analysis, causal effect inference, mortality prediction, etc. However, whereas the EHR data warehouses are usually enormous, a common setback often met by bioinformatics researchers is that populations quickly become scarce when restricted to cohorts of interest, rendering almost impossible using the raw high-dimensional data. To that extent, several attempts have been made in learning general-purpose representations from patient records, to make downstream predictions easier and more accurate.

% These records usually contain a large set of numerical features such as patient demographics (e.g. age, gender, ethnicity), lab measurements (e.g. blood gases, fluid balances, vital signs), binary indicators for diseases and medical procedures, as well as free-text clinical notes. While numerical fields can be straightforward to use in most machine learning models, there is no common ground on how to process clinical notes from physicians and nurses. Researchers often use general-purpose off-the-shelf techniques, such as fitting topic models or learning direct word representations. These techniques, besides being somewhat impractical from a computational standpoint, are very generic and do not leverage the particular structure of these notes. They are, for each patients, a sequence of un-ordered collections of words\footnote{The words are always un-ordered in the notes as a consequence of the anonymization and annotation pipeline in the annotator used in our dataset, which is quite widely spread.}.

==> unused/methods_old.tex <==
\section{Methods}

We explore three types of methods, which we explain here. They are, respectively, learning word-level embeddings and aggregating them to a fixed-length representation, fitting a sequence model to patients' notes to learn all embeddings jointly, and  learning a cross-channel encoder from medical notes to diagnoses.

% We also start by presenting the baseline we will use in our experiments.

% \subsection{Baseline}

% For evaluations involving predictions (at the note and patient level), we use a simple bag-of-words as a baseline, where the vocabulary is restricted to the words present in the training set. This represents about 30k words (to evaluate our embeddings in a realistic setting, we train the evaluation tasks on small datasets).

% Since such high dimensionality causes practical issues (runtime, convergence, \dots) we also consider selecting only the 15,000 words being most represented in the patients record (in terms of number of unique patients per word). This restriction was unavoidable in order to fit a logistic regression (\texttt{glmnet} with L2 regularization) with 2,000 training patients.

\subsection{Embed and aggregate}
% Our first proposed method is learning embeddings at the word level, before aggregating them at the note and patient level.
We first propose a method to learn word embeddings from clinical notes, and then discuss how these can be aggregated to represent a note or a patient state. 

\subsubsection{Learning word embeddings from clinical notes}

It is natural to think about common methods in Natural Language Processing to learn word embeddings, such as \texttt{GloVe}\cite{pennington2014glove} and \texttt{Word2Vec}\cite{mikolov2013distributed}. However, as explained above, the Open Biomedical Annotator removes the order of words in the notes as part of the de-indentification process. We decided to tackle this challenge by simply re-generating notes with a random word order. Such approach was already proposed (e.g. in \cite{choi2015doctor} and \cite{choi2016learning}) as an easy trick to deal with the unordered medical codes and did not seem to alter the models' quality. However since clinical notes can be quite long, we suspect that it might be too hard for our models to capture the context of a word. Therefore, we also propose to juxtapose a couple times duplicates of a same note, but with different random orders. 

This makes our data look exactly like text data, so that we can learn embeddings with  an efficient C implementation of GloVe\footnote{\url{https://github.com/stanfordnlp/GloVe}}.

\subsubsection{Learning word embeddings from external data (MCEMJ)}
\label{sec:mcemj}

In \cite{de2014medical} the authors learn embeddings from 350,000 medical journal abstracts in the OHSUMED dataset. They first map the free text to UMLS\footnote{Unifieid Medical Language System, the same as the one we use.} concept ID's and then learn the word embeddings using Word2Vec’s skip-gram model with hierarchical softmax. Their best results were achieved with embeddings of dimension 200 and a window size of 5. 52,100 such embeddings were shared publicly by the authors \footnote{\url{https://github.com/clinicalml/embeddings}} and approximately 28,000 of them belonged to our vocabulary. We will refer to them as MCEMJ (Medical Concept Embeddings from Medical Journal).

\subsubsection{Fixed-length aggregation at the note and patient level}
Although it seems to be a simple approach, it is still very common in medical applications to aggregate a patient's data over time by summing or averaging counts of medical codes. Similarly, we propose to aggregate (mean, max, min, or sum) the word embeddings per note and then per patient. We explored these various ways of pooling the embeddings both on the note and the patient level.

In addition, we investigate the utility of concatenating multiple of these  patient-level aggregations, especially some derived by different sources of embeddings (e.g. randomly ordered notes and medical journals).

\subsection{Recurrent neural network}

Our methods so far do not rely on the sequential nature of the notes in a patient's history. For a number of prediction tasks, it is important to capture the progressive evolution of a patient's state in its representation. Thus, it is a natural idea to use recurrent neural networks to learn those patient-level embeddings. 
% For each patient (or batch of patients), we feed the ordered notes a sequence.

\subsubsection{Supervision}

We supervise our network with diagnoses associated with the notes (from the corresponding \textit{visits}, as explained in \ref{sec:pres}). Since these descriptors are extremely high-dimensional, we map them to more general disease categories using the Clinical Classification Software (CCS)\footnote{https://www.hcup-us.ahrq.gov/toolssoftware/ccs/ccs.jsp}, leaving a label space of dimension 254. 

At this point we have a design choice, training the network as a multi-task sequence classification problem (aggregating the CCS labels on a per-patient basis), or as a sequence labeling problem (supervising each timestep with its corresponding CCS codes). Experiments showed that the former gave considerably higher scores on the evaluation task, which is a probable consequence of the labels' sparsity (the latter providing very scarce supervision signal).

\subsubsection{Architecture}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{rnn.png}
\caption{Model architecture}
\end{figure}

\textbf{Pooled embedding layer}

Since this un-ordered structure in the input is quite uncommon, we use an unusual layer as input to our neural network. This layer computes trainable embeddings from the collections of words in an input note, and pools them before feeding them to the rest of the network. More precisely, we use max-pooling aggregation, so the input to our network for a note $x$ is actually given by:

$$ \phi_L(x) = \text{max}_1(x \odot  L) $$

where $x=[0,0,1, ... ,0,1,0]$ is the note bag-of-words encoding of shape $(V,1)$, $L$ is the word embedding matrix of shape $(V, D_x)$ ($V$ being the vocabulary size and $D_x$ the word embedding size), and $\text{max}_1$ performing a max over the first dimension.

We also explored with aggregating the word embeddings by taking their average, but this performed extremely poorly on the evaluation tasks. It makes sense to use particularly activated features in the learned word representations rather than their average, as those activated features will capture specific semantic indicators from the note.

\textbf{RNN cells}

We explored both using Long Short-Term Memory (\cite{hochreiter1997long}) and Gated Recurrent Units (\cite{cho2014learning}) as cell structure for our recurrent network. We found that LSTM learned a poor representation of the input, leaving a number of columns at 0 and performing poorly on evaluation tasks, which confirms the findings of \cite{choi2015doctor}. Thus, most of our final experiments were conducted with GRUs, and this is what we strongly recommend for researchers working with similar problems. \\

\textbf{Other details} 

We used \texttt{tanh} activations, dropout (with drop probability 0.1 or 0.2 depending on models), and a dense layer with binary cross-entropies for the multi-task supervision. We trained the networks for 100 epochs, using RMSProp (\cite{tieleman2012lecture}) for loss optimization. The models were implemented in Keras (\cite{chollet2015keras}) and trained on a NVIDIA GeForce GTX TITAN X GPU.

\subsubsection{Embeddings initializations}

We explored initializing our embeddings in various ways. In particular, we tried initializing them randomly, with word embeddings pre-trained on our notes, and with word embeddings trained on journal abstract (MCEMJ) (see \ref{sec:mcemj} for details). While the results for random initialization and MCEMJ initialization are reported below, we found that initializing the weights with embeddings pre-trained on the clinical notes themselves gave very poor results on the evaluation tasks.


\subsection{Note-level cross-channel autoencoder}

Finally, we experimented with a flat version of the sequential model presented in the previous section, \textit{ie.} a two-hidden-layer neural network where the first layer is a randomly initialized embedding layer with max-pooling. For this model, the inputs are the clinical notes and the non-exclusive targets are CCS labels derived from the corresponding visit data.

This model seems appealing since it leverages our data to provide supervision in order to learn word embeddings. In addition, it is simpler to implement and deploy than a sequential model. However we found that in practice it mostly combined the drawbacks of both previous models: it does not provide a clear patient-level representation, it requires a lot of training data (and labels!), and is also very slow to run.

